Sandwiching Random Geometric Graphs and Erdos-Renyi with Applications: Sharp Thresholds, Robust Testing, and Enumeration

The distribution $\mathsf{RGG}(n,\mathbb{S}^{d-1},p)$ is formed by sampling independent vectors $\{V_i\}_{i = 1}^n$ uniformly on $\mathbb{S}^{d-1}$ and placing an edge between pairs of vertices $i$ and $j$ for which $\langle V_i,V_j\rangle \ge \tau^p_d,$ where $\tau^p_d$ is such that the expected density is $p.$ Our main result is a poly-time implementable coupling between Erd\H{o}s-R\'enyi and $\mathsf{RGG}$ such that $\mathsf{G}(n,p(1 - \tilde{O}(\sqrt{np/d})))\subseteq \mathsf{RGG}(n,\mathbb{S}^{d-1},p)\subseteq \mathsf{G}(n,p(1 + \tilde{O}(\sqrt{np/d})))$ edgewise with high probability when $d\gg np.$ We apply the result to: 1) Sharp Thresholds: We show that for any monotone property having a sharp threshold with respect to the Erd\H{o}s-R\'enyi distribution and critical probability $p^c_n,$ random geometric graphs also exhibit a sharp threshold when $d\gg np^c_n,$ thus partially answering a question of Perkins. 2) Robust Testing: The coupling shows that testing between $\mathsf{G}(n,p)$ and $\mathsf{RGG}(n,\mathbb{S}^{d-1},p)$ with $\epsilon n^2p$ adversarially corrupted edges for any constant $\epsilon>0$ is information-theoretically impossible when $d\gg np.$ We match this lower bound with an efficient (constant degree SoS) spectral refutation algorithm when $d\ll np.$ 3) Enumeration: We show that the number of geometric graphs in dimension $d$ is at least $\exp(dn\log^{-7}n)$, recovering (up to the log factors) the sharp result of Sauermann.

==> Introduction.tex <==
\section{Introduction}

Random graphs have been a fundamental object of study since the seminal paper of Erd{\H o}s and R\'enyi \cite{Erdos1959ER}. In the \ERspace model $\ergraph,$ each edge among $n$ vertices appears independently with probability $p.$ This model has been instrumental to major developments in combinatorics, algorithm design and complexity, and network modeling.  

Both theory and practice have led researchers more recently to consider models in which edges are not independent but are rather a (random) function of (random) feature vectors of the nodes. Such models oftentimes exhibit dependence between edges. For instance, one common set-up is when feature vectors belong to a metric space and the probability of an edge between two nodes increases as the distance between vectors decreases. The axiomatic triangle inequality leads to a large occurrence of triangles in such graphs, a phenomenon referred to as ``the friend of my friend is also a friend of mine.'' A concrete model of interest is the \emph{Spherical Random Geometric Graph}. 

\begin{definition}
\label{def:sphericalrgg}
The spherical random geometric graph $\RGGsphere$ on $n$ vertices $[n] = \{1,\ldots, n\}$ of
dimension $d$ with expected density $p$ is defined as follows. First, $n$ vectors $V_1,  \ldots, V_n$ are drawn independently from the uniform distribution on the sphere $\dsphere.$ Then, an edge between $i$ and $j$ is formed if and only if $\langle V_i ,V_j\rangle \ge \tau^p_d.$ Here, $\tau^p_d$ is chosen so that $p = \prob[\langle V_i ,V_j\rangle \ge \tau^p_d].$ 
\end{definition}


Reasons to study random geometric graphs together with prominent examples include:
\begin{enumerate}
    \item \emph{Understanding the Role of Independence in Combinatorial Phenomena:}  
    \cite{goel05monotoneproperties} show that random geometric graphs in sufficiently low dimension (when very strong dependence between edges is present) exhibit \emph{sharp-thresholds phenomena}. This extends one of the milestone results on \ERspace graphs to non-product distributions.  
    \item \emph{Combinatorial Constructions:} Dependence between edges may give rise to combinatorial properties not shared by the more common \ERspace model. \cite{Liu22Expander} show that in certain regimes of a low (logarithmic) dimension random geometric graphs are 2-dimensional expanders (an object for which no other randomized construction was known prior to their work).
    % \cite{Devroye11} show that the clique number of a (sufficiently high-dimensional) random geometric graph nearly matches the clique number of \ERspace  at the same density (even in a regime when the two distributions are at a $1 - o(1)$ total variation distance from each other). 
    \item \emph{Statistical Inference With Dependent Data:} Random geometric graphs provide a convenient model for developing tools for learning and estimation from dependent data. Lack of independence makes inference much more challenging but also more realistic due to the non-iid nature of real-life networks. 
    %Several questions of interest have been studied. 
    Can one even test for dependence, i.e. test between a random geometric graph and \ERspace \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}? Can one estimate the dimension of the latent vectors \cite{Bubeck14RGG}? Can one recover the latent vectors \cite{li2023spectral} from the graph?    
    \item \emph{Modeling Real-Life Networks:} The edge probabilities in social, biological, communication networks depend on features of the entities represented by nodes. Theoretical and empirical results show that geometric graphs fit well certain properties of brain networks \cite{vempala23kcap}, social networks \cite{Almagro22}, and protein-protein interaction networks \cite{higham08}. \textbf{Remark:} We do not claim that any concrete model such as \cref{def:sphericalrgg} fits the data perfectly. This is an important point that we will return to.
\end{enumerate}

Comparing $\RGGsphere$ and $\ergraph$ in total variation, which is the focus of the majority of the existing works on \emph{high-dimensional} random geometric graphs thus far, is an important benchmark question. 
Yet, it does not capture key aspects of the four directions outlined.

% In the current work, we also compare $\RGG$ and \ERspace but   Such a relaxation is motivated by all four reasons to study random geometric graphs that we outlined. 

Understanding combinatorial phenomena in graphs with dependence between edges explicitly requires the distribution to \emph{not be} \ER. Statistical tasks in non-iid settings (beyond testing for independence) also require a distribution other than \ER. Finally, when modeling complex networks, it is too much to hope that all edges are explained by a simple generative model such as the one in \cref{def:sphericalrgg}. Even ignoring the simplicity of the threshold function $\indicator[\langle\cdot,\cdot\rangle\ge \tau^p_d],$ edges are only determined by pairwise compatibility of the feature vectors and higher-order effects are not captured. Additionally, in real-life networks, (potentially adversarial) corruptions might be present due to malicious entities or non-uniform errors in measurements. Again, testing in total variation is not the correct framework in the presence of corruptions. 

% For example, in social networks, the probability of a friendship may depend on a large variety of factors such as age, geographic location, education, occupation... \footnote{Even though, by no means we claim that any such set of factors fully determines whether there is a friendship. This is an important point that we will return to.} Correlations  

% Random graphs with underlying geometric structure are not only more realistic in modelling real-life networks, but also
% provide a fruitful counterpart to the well-studied \ER model for theoreticians. The dependence among edges leads to genuinely novel combinatorial phenomena (not shared by the simpler \ER model). At the same time, it also makes associated learning and estimation tasks in a non-iid setting much more challenging (but also more realistic due to the non-iid nature of real-life networks).



% Random geometric graphs in low dimension have been extensively studied (see \cite{penrose03} and references therein). The study of the high-dimensional regime in which $d$ grows with $n,$ potentially even at a polynomial rate, however, was more recently initiated by 
% \cite{Devroye11}. In \cite{Devroye11}, the authors discuss both \emph{combinatorial properties} of the distribution, concretely the typical size of the largest clique, as well as \emph{statistical tasks}, namely testing between a random geometric graph and \ER with a single sample. Since then, both directions have flourished. . Determining the regime in which the testing problem is information theoretically possible is still open even though it has witnessed continuous progress  Other statistical tasks have also been studied such as dimension estimation \cite{Bubeck14RGG} and recovering the latent vectors from the graph data \cite{li2023spectral}.  

\subsection{Our Results} 
  These reasons call for  
  a less stringent than total variation comparison between \ERspace and random geometric graphs. 
  We study the following \emph{approximate stochastic dominance}
  (see \cref{thm:stochasticcoupling} and \cite{Liu2022STOC}):
\begin{equation}
\label{eq:couplinquestion}
\tag{Q1}
\begin{split}
    &\textit{When can one couple the two graph distributions in such a way that with high probability}\\
    &\quad\quad\quad\quad\quad\mathsf{G}(n,p(1-\epsilon))\subseteq \RGGsphere \subseteq\mathsf{G}(n,p(1+\epsilon))\textit{ for some small } \epsilon?
    \end{split}
\end{equation}
Here, inclusion is over the edge set. 
Such a coupling \emph{captures simultaneously monotonicity and robustness}.  enables us to address aspects of all four of the aforementioned directions:
\begin{enumerate}
    \item \emph{Understanding the Role of Independence in Combinatorial Phenomena:} We use the \emph{edge-monotonicity} of the coupling to compare monotone properties of $\ergraph$ and $\RGGsphere.$ We give the first proof of sharp thresholds for monotone properties of $\RGG$ in a non-trivial high-dimensional regime.
    \item \emph{Combinatorial Constructions:} A coupling of the form in \cref{eq:couplinquestion} implies a lower bound on the support size of the $\RGGsphere$ distribution. This allows us to use $\RGGsphere$ as a randomized construction for 
    counting the number of geometric graphs in dimension $d.$ 
    \item \emph{Statistical Inference With Dependent Data:} One view of a coupling of the form in \cref{eq:couplinquestion} is that a sample of $\ergraph$ is a sample of $\RGGsphere$ with $O(\epsilon n^2 p)$ adversarially corrupted edges. This leads us to consider the well-studied question of testing between $\ergraph$ and $\RGGsphere$ \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier} in the previously unexplored setting of adversarial edge-corruptions.  
    \item \emph{Modeling Real-Life Networks:} More generally, random geometric graphs with bounded (but otherwise arbitrary) edge corruptions more accurately model real-life networks due to the potential presence of edges not explained by the geometry. 
\end{enumerate}

\subsubsection{Main Theorem and Interpretation}
% Motivated by the last consideration -- model mis-specifications and adversarial corruptions -- we choose to study a comparison which allows for a fraction of unexplained edges. Our main theorem is the following algorithmic result.

\begin{theorem}[Main Coupling Result]
\label{thm:algorithmiccoupling}
Consider some $n,d,p$ such that $d= \Omega( \max(np,\log n))$ and $p = \Omega(1/n), p\le 1/2.$ There exists a polynomial-time algorithm which on input $H\sim \ergraph,$ outputs $n$ vectors $V_1 = V_1(H), V_2 = V_2(H), \ldots, V_n = V_n(H)$ in $\dsphere$ with the following two properties:
\begin{enumerate}
    \item The marginal distribution of the vectors is independent uniform: $V_1, V_2, \ldots, V_n\iidsim\unif(\dsphere).$
    \item With high probability (over the input and internal randomness), $\indicator[\langle V_i, V_j\rangle\ge \tau^p_d] = H_{ij}$ for all pairs $i,j$ such that $|\langle V_i, V_j\rangle - \tau_p^d|\ge \frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{3/2}}{d}$ for some absolute constant $c.$
     
\end{enumerate}
\end{theorem}
In other words, the algorithm described above couples $\RGG$ and $\ergraph$ in such a way that they only differ at pairs $(i,j)$ for which $\langle V_i, V_j\rangle $ is very close to the threshold. Elementary calculations shows that with high probability, $G,H$ differ at only $\tilde{O}\Big(\binom{n}{2}p\times\sqrt{\frac{{np}}{d}}\Big) = o\Big(\binom{n}{2}p\Big)$ edges. An immediate implication of \cref{thm:algorithmiccoupling} is the following approximate  stochastic dominance. 

\begin{corollary}[Approximate Stochastic Dominance]
\label{thm:stochasticcoupling}
Consider some $n,d,p$ such that $d= \Omega(np\log^4 n, \log^5n)$ and $p = \Omega(1/n).$ Then, there exists a coupling of $G\sim\RGG(n,\dsphere,p),$ $H_-\sim \mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ and $ H_+\sim \mathsf{G}(n,p(1+\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})),$ 
 such that 
$$
H_-\subseteq G \subseteq H_+
$$
with high-probability, where inclusion is defined as inclusion over the edge set.
\end{corollary}

In \cite{Liu2022STOC}, the authors prove \cref{thm:stochasticcoupling} under the weaker condition $d \ge \polylog(n)\times n^2p^2$ with the purpose of describing the local structure of random geometric graphs. Our stronger result, based on an entirely different proof technique, is crucial for some of the applications to follow.

Note that $d =\tilde{\Theta}(np)$ is a polynomially smaller dimension than the one required for\linebreak $\TV(\RGGsphere, \ergraph) = o(1),$ For the latter statement to hold, $d= \tilde{\Omega}(n^3p^3)$ is needed as demonstrated by the signed triangle count test \cite{Bubeck14RGG,Liu2022STOC} which is also conjectured to be optimal \cite{Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}. While $d = \tilde{\Theta}(n^3p^3)$ is still rather mysterious, the critical dimension in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} $d = \tilde{\Theta}(np)$ has two natural coalescent interpretations:
\begin{enumerate}
    \item \textbf{Entropic Threshold:} The maximal entropy of a graph with expected density $p$ is $\binom{n}{2}H(p) = \tilde{\Theta}(n^2p)$ and this is achieved by $\ergraph.$ On the other hand, the following heuristic (which we make rigorous in \cref{sec:enumeration}) suggests that the entropy of $\RGGsphere$ is at most $\tilde{\Theta}(nd).$  $\dsphere$ has an $\epsilon$-net of size $\exp(\tilde{O}(d\log(1/\epsilon))).$ 
    Hence, we can discretize the sphere into $\exp(\tilde{O}(d))$ points. As there are $n$ latent vectors $V_1, V_2, \ldots, V_n,$ each effectively of the $\exp(\tilde{O}(d))$-discretization, and the latent vectors uniquely determine the geometric graph, the $\RGGsphere$ distribution effectively has support size 
    $\exp(\tilde{O}(nd)).$ Hence, its entropy is at most $\tilde{O}(nd).$ To match (up to lower order terms) the $\tilde{\Theta}(n^2p)$ entropy of $\ergraph,$ one therefore needs $d = \tilde{\Omega}(np).$ Using \cref{thm:algorithmiccoupling}, in \cref{sec:enumeration} we show that when $d = \tilde{\Omega}(np),$ the support size of $\RGGsphere$ is indeed ``maximal'', i.e. of size $\exp(\tilde{\Omega}(n^2p)).$
    \item \textbf{Spectral Threshold:} Miraculously, as soon as $d \lesssim np,$ there is a spectral separation between $\ergraph$ and $\RGGsphere.$ 
    The second largest eigenvalue of $\ergraph$ is $\tilde{\Theta}(\sqrt{np})$ while the second largest eigenvalue of $\RGGsphere$ is 
    $\tilde{\Theta}({\frac{np}{\sqrt{d}}})\gg \tilde{\Theta}(\sqrt{np})$
    \cite{Liu22Expander,li2023spectral}.
    This spectral separation allows for efficient spectral and SDP algorithms, as in \cite{li2023spectral} and \cref{sec:robusttesting}.
\end{enumerate}

% We will get back to this point in \cref{sec:discussion}, but we believe that the coincidence of entropic and spectral thresholds for the $\RGGsphere$ distributions heuristically explains why no information-computation gaps have been observed for natural statistical tasks such as testing, robust testing, and embedding of random geometric graphs. As soon as there is a very strong information theoretic separation between $\RGG$ and $\ergraph,$ there is also a computationally efficient (spectral) witness.

\begin{remark} We note that in general a relaxed stochastic dominance of the form in \cref{thm:stochasticcoupling} does not guarantee closeness in total variation even if one couples 
$H_-\sim \mathsf{G}(n,p), H_+\sim \mathsf{G}(n,p), G\sim\mathcal{D}$ such that $H_-\subseteq G\subseteq H_+$ with high probability for some $\mathcal{D}.$ Specifically, consider a distribution $\mathcal{D}$ defined by the following coupling. $H_-$ is drawn from $\ergraph.$ Then, $H_+$ is a copy of $H_-$ except that a uniformly random non-edge is changed to an edge. One can check that whenever $p= \Omega(1/n),$ the distribution of $H_+$ is only $o(1)$ TV distance away from $\ergraph.$ Finally, $G$ is the graph among $H_-, H_+$ with an even number of edges. Clearly, $H_-\subseteq G\subseteq H_+$  w.h.p. but $\TV(\mathcal{D}, \ergraph) \ge 1/2 - o(1)$ as the distribution $\mathcal{D}$ is supported on graphs with an even number of edges.
\end{remark}

\subsubsection{Application I: Robust Testing} One immediate application of \cref{thm:stochasticcoupling} is  the following. Suppose that 
$\epsilon\in (0,1]$ is a small fixed constant. Whenever $d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5)$ (where $K(\epsilon)$ depends solely on $\epsilon$), one can with high probability (adversarially) corrupt $\epsilon \binom{n}{2}p$ edges of a sample from $\RGGsphere$ and produce a sample from $\ergraph.$
Hence, the following robust testing problem is information-theoretically impossible when $d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5):$ 
\begin{problem}[Robust Testing of Geometry With Edge Corruptions]
\label{problem:robusttesting}
Given are $n,d\in \mathbb{N},$ $p\in [0,1]$ and a fixed constant $\epsilon.$
Consider the following hypothesis testing problem. One observes a graph $H$ and needs to decide between $H_0: H = \mathcal{A}(\bfG),\bfG\sim \ergraph$ and 
$H_1: H = \mathcal{A}(\bfG),\bfG\sim \mathsf{RGG}(n,d,p).$ Here $\mathcal{A}$ is an arbitrary adversary who is allowed to corrupt at most $\epsilon \binom{n}{2}p$ edges and non-edges.
\end{problem}
We restrict the adversary to changing $\epsilon \binom{n}{2}p$ edges for a small constant $\epsilon$ as the robust testing problem is otherwise trivially impossible. Both $\mathsf{RGG}(n,d,p)$ and 
$\ergraph$ have with high probability $1.5\binom{n}{2}p$ edges. Hence, an adversary $
\mathcal{A}$ who simply deletes all edges of a sample from $\RGG$ and then inserts Bernoulli $p$ edges (in total $3\binom{n}{2}p$ w.h.p.) can transform into a sample from $\ergraph.$ Hence, \cref{problem:robusttesting} captures the setting of ``maximal adversaries.'' 

\begin{remark}[Efficient adversaries]
\label{rmk:eficientadversary}
When $d = o((np)^3(\log n)^3), d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5)),$ \cref{problem:robusttesting} is information theoretically impossible even against polynomial-time adversaries. In this regime, an adversary can see a sample $H$ and (correctly with high probability) test using the signed-triangle statistic \cite{Liu2022STOC} whether the sample is from $\ergraph$ or $\RGGsphere.$ If $H$ is from $\ergraph,$ the adversary can use the efficient algorithm from \cref{thm:algorithmiccoupling} and produce (with high-probability) a sample from $\RGGsphere$ differing from $H$ only at $o\Big(\binom{n}{2}p\Big)$ edges. If $H$ is from $\RGG$ already, the adversary does not change edges. 
\end{remark}



Due to the miraculous coincidence of spectral and entropic thresholds, \cref{problem:robusttesting} is solvable in polynomial time even against computationally unbounded adversaries when $d\ll np.$ 

\begin{theorem}
\label{thm:robustestingsos}
There exists some constant absolute constant $K_r>0$ with the following property. When $d\le K_r\min(np\log(1/p), n^2p^2\log(1/p)\log^{-2}n)$ and $d = \omega(\log 1/p),$ there exists a polynomial-time algorithm solving \cref{problem:robusttesting} with high probability for all $\epsilon\le K_r.$
\end{theorem}
We overview the algorithm in \cref{sec:nontechnicalrobust} and give full detail in \cref{sec:robusttesting}. It is a constant degree SoS program for spectral refutation of a small operator norm of the centered adjacency matrix. The key insight, implicit in \cite{li2023spectral}, is that the latent vectors witness a large second eigenvalue for a random geometric graph. The approach works for robust testing against any null hypothesis with a substantially smaller second eigenvalue than $\RGGsphere,$ see \cref{rmk:testingrobustly}.

\begin{remark}
\label{rmk:couplingimpossibilityfromspectral}
\cref{thm:robustestingsos} implies that when $d \le K_r\min(np\log(1/p), n^2p^2\log(1/p)\log^{-2}n),$ there does not exist a coupling between $H_-\sim \mathsf{G}(n,p(1-o(1)),G\sim \RGGsphere, H_+\sim \mathsf{G}(n,p(1+o(1))$
such that $H_-\subseteq G\subseteq H_+$ w.h.p. Otherwise, one can use this coupling as an adversary for \cref{problem:robusttesting} even against computationally-unbounded testers but \cref{thm:robustestingsos} shows that such an adversary cannot exist. Hence, the dimension requirement $d = \tilde{\Omega}(np)$ in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} is tight (up to $\polylog$ factors).
\end{remark}

\subsubsection{Application II: Sharp Thresholds} The coupling in \cref{thm:stochasticcoupling} between random geometric graphs and \ERspace is monotone in the sense that 
$
H_-\subseteq G \subseteq H_+.
$
Whenever $H_-\sim \mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ satisfies an increasing property with high probability, so does $G\sim \RGGsphere.$ Whenever 
$G\sim \RGGsphere$ satisfies an increasing property, so does $H_+\sim \mathsf{G}(n,p(1+\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})).$ 
This immediately allows us to translate sharp-threshold phenomena from \ERspace to RGG by considering the couplings between $G_-\subseteq H_-$ 
where 
$G_-\sim \RGG(n,\dsphere,p(1-3\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ and  
$H_+\subseteq G_+ $ where
$G_+\sim \RGG(n,\dsphere,p(1+3\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})).$

\begin{theorem} Suppose that $\mathcal{P}_n$ is a monotone property with critical probability $p^c_n$ which satisfies $p^c_n = \Omega(1/n).$ 
Suppose further that $\mathcal{P}_n$ exhibits a sharp threshold with respect to $\ergraph$ and has a critical window of length $\omega_\epsilon = o(p^c_n).$ 
If $d_n=  \omega(\max(np^c_n\log^4 n, \log^5n)),$ the property $\mathcal{P}_n$ also exhibits a sharp threshold with respect to $\RGG(n,d_n,p)$ and has critical probability $p^c_n + O\Big(p_n^c\frac{\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}\Big)$ and critical window of length 
$\omega_\epsilon  +  O\Big(p_n^c\frac{\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}\Big).$
\end{theorem}

This theorem partially answers in the affirmative a question due to Perkins on whether high-dimensional random geometric graphs exhibit sharp thresholds \cite{perkins2024searching}. 

\subsubsection{Application III: Enumeration}  \cref{thm:stochasticcoupling} demonstrates that $\RGGsphere$ is a distribution over at least $\exp(\tilde{\Omega}(n^2p))$ graphs when $d= \max(np\log^4 n, \log^5 n).$ The proof is rather simple - if $\mathcal{M}$ is the support of $\RGGsphere,$ using a simple counting argument one can bound the number of graphs that are edge-subgraphs of some graph $H$ in $\mathcal{M}$ and differ from $H$ in $o(\binom{n}{2}p)$ edges. Using this bound, one can arrive at an upper bound for the entropy of $\mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ (which is $\tilde{\Theta}(n^2p)$).  This, in turn, implies a lower bound on $|\mathcal{M}|.$ Altogether, this gives the following result.

\begin{theorem}
\label{thm:enumeration}
The number of graphs which can be realized as intersection graphs of unit spheres in dimension $d$ is at least $\exp(nd\log^{-7}n).$     
\end{theorem}

The statement is tight up to the $\log$ terms as shown in \cite{SAUERMANN2021107593}. The result is not new and sharper estimates (up to the log terms) were recently shown in \cite{SAUERMANN2021107593}. Nevertheless, one advantage of our proof is its simplicity - it is based on a natural probabilistic construction, spherical random geometric graphs. The techniques from algebraic geometry and algebraic topology in \cite{SAUERMANN2021107593} are significantly more involved, even though admittedly much more systematic and sharper.

\subsection{Prior Work and Challenges}
\paragraph{Coupling Random Geometric Graphs and \ER.} In \cite{Liu2022STOC}, the authors prove \cref{thm:stochasticcoupling} under the weaker condition $d\ge n^2p^2\log^4n.$ In their construction, they sample $V_1, V_2, \ldots, V_n$ sequentially. A caricature of their argument is that with high probability, when sampling $V_1, V_2, \ldots, V_{k-1}$ the intersection of any $i\approx pk$ $p$-caps and $k-i-1\approx k(1-p)$ $p$-anti-caps corresponding to $V_1, V_2, \ldots, V_{i-1}$\footnote{For $V\in \dsphere,$ the associated $p$-cap is the set $\{U \in \dsphere\; : \langle U, V\rangle\ge \tau^p_d\}$  and the $p$-anti-cap is its complement} is sufficiently close to $p^{i}(1-p)^{k-i-1}.$ Hence, one should expect that the edges from $k$ to $[k-1]$ roughly are distributed as ``independent'' $\Bernoulli(p)$ variables. They make this statement precise by quantifying ``sufficiently close'' via a concentration argument based on transportation inequalities. While our proof of \cref{thm:stochasticcoupling} is entirely different, it suggests what might be suboptimal in the approach of \cite{Liu2022STOC}. Typical intersections of $\approx pk$ caps and $k-i-1\approx k(1-p)$ anti-caps might concentrate much better than worst-case 
intersections due to a square-root cancellation phenomenon. We use this idea in our proof to get $d\ge \max(np, \log n)$ and if we consider \emph{all} intersections of caps and anti-caps instead, we also obtain a result for $d\ge n^2p^2\polylog n.$ While the square-root cancellation comes naturally in our martingale-based analysis, it is unclear whether it can be incorporated in the transportation-based approach of \cite{Liu2022STOC}. Even beyond that, an advantage of our approach is that there is an efficient algorithm producing the coupling -- \cref{thm:algorithmiccoupling}. The result of \cite{Liu2022STOC} is not obviously algorithmically efficient as it requires keeping track of an intersection of caps and anti-caps on the sphere and being able to sample and estimate the volume of this intersection.    

A different work which shows that in certain regimes random geometric graphs can be represented as $\ergraph$ with some planted structure (i.e. the edges on locations for which $|\langle V_i, V_j\rangle - \tau_p^d|\le \frac{\sqrt{np\log n}}{d}$ in \cref{thm:algorithmiccoupling}) is 
\cite{bangachev2024fourier}. In fact, in their representation, again the non-\ERspace pairs $(i,j)$ are exactly the ones for which $\langle V_i, V_j\rangle$ are close to $\tau^p_d$ (called \emph{fragile pairs} in \cite{bangachev2024fourier}). While some of our ideas are related to and motivated by \cite{bangachev2024fourier}, there is a fundamental barrier to their proof technique. It crucially relies on performing the Gram-Schmidt operation on the latent vectors\footnote{To be fully precise, the Gram-Schmidt is performed on the isotropic Gaussian vectors $Z_1, Z_2, \ldots, Z_n.$ 
% where $Z_i = V_i \chi_i$ (where $\chi_i$ is an appropriate square root of a $\chi^2$ random variable). 
This, however, makes little difference to the arguments in \cite{bangachev2024fourier} and the current work, see \cref{rmk:sphericaltogaussian}.} $V_1, V_2, \ldots, V_n.$ In particular, this method requires $d\ge n,$ so obtaining a result of the form in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} for $d\ll n$ is impossible. 

\paragraph{Testing.} To the best of our knowledge, this work is the first to study the robust testing problem between $\RGGsphere$ and \ER. The same question in the setting of no edge corruptions has attracted significant attention in recent years \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}. Formally, one observes a graph $G$ and needs to decide $H_0:G\sim \ergraph$ or $H_1:G\sim \RGGsphere.$ By counting signed triangles, i.e computing $\sum_{i<j<k}(G_{ij} - p)(G_{jk}-p)(G_{ki}-p),$ one can succeed with high probability whenever $d = \omega(n^3p^3\log^3(1/p))$ \cite{Bubeck14RGG,Schramm_2022}.  The current state-of-the-art information-theoretic lower bounds are that when $d\ge (\log n)^C n^3p^2,$ the problem is information theoretically impossible as well as when 
$p = \Theta(1/n)$ and $d\ge (\log n)^C$ for some constant $C$ \cite{Liu2022STOC}. Even ignoring $\polylog $ factors, there is still a $1/p$ gap between the testing algorithm and the information-theoretic lower bound when $1/n\ll p\ll 1/2.$ The gap was recently closed with respect to low-degree polynomial tests by \cite{bangachev2024fourier}. Counting signed triangles is optimal among all degree $\log^{2-\epsilon} n$ polynomial tests.

We note that both the question of upper and lower-bounds are significantly different when one considers the testing problem with a constant number of adversarial corruptions \cref{problem:robusttesting}. On the algorithmic side, simple counting tests such as counting signed triangles necessarily fail. For example, the expected number of signed triangles in $\RGGsphere$ is $\tilde{\Theta}(n^3p^3/\sqrt{d})$ \cite{Liu2022STOC}. One can increase the expected number of signed triangles in $\ergraph$ by planting a clique of size $\tilde{O}(np/d^{1/6})$ which requires $\tilde{O}(n^2p^2/d^{1/3}) = o(n^2p)$ adversarial corruptions. One can argue similarly for other subgraph-counting tests. This is why we need a more sophisticated sum-of-squares spectral refutation algorithm which uses the true embedding as a witness. To the best of our knowledge, \cite{mao2024informationtheoretic} is the only other work which uses an embedding-based approach for testing for random geometric graphs, but their work is in low-dimension and the algorithm is not computationally efficient. Regarding lower-bounds, all of the prior work on the setting without adversarial corruptions \cite{Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC} very strongly exploits distributional assumptions (such as the relationship to Wishart ensembles and a certain $\KL$-convexity argument revealing the latent vectors). We do not expect that any of these techniques applies to the adversarial setting. Instead, we rely on our coupling argument \cref{thm:stochasticcoupling}.

Finally, there is still a gap between the known upper-bound $\tilde{\Theta}(n^3p^3)$ and the lower-bound $\Tilde{\Theta}(n^3p^2)$ in the setting of no corruptions when $p = \omega(1/n).$ In this work, we determine that (up to log factors) $d = \Tilde{\Theta}(np)$ is the tight threshold for testing with adversarial corruptions computationally and information-theoretically. Part of the reason for this difference between the robust setting and the setting without corruptions is how well we understand the respective thresholds. $d = \Tilde{\Theta}(np)$ has a very clear significance - as an entropic threshold information-theoretically and as a spectral threshold computationally. Yet, the condition $d = \Tilde{\Theta}(n^3p^3)$ so far seems to only have a computational interpretation. It is the threshold below which one can test counting signed triangles, which are ``the most informative subgraph'' among $\log^{2-\epsilon}n$-sized subgraphs \cite{bangachev2024fourier}. The search for the correct information-theoretic interpretation of  $d = \Tilde{\Theta}(n^3p^3)$ remains open.

\paragraph{Sharp Thresholds.} The question of whether monotone properties exhibit sharp thresholds is by far the best understood in the case of product distributions. The seminal paper of \cite{Friedgut1999SharpTO} establishes very broad conditions on vertex-transitive properties for which the \ERspace distribution exhibits sharp-thresholds. In non-product settings, much less is understood. Important progress has been made in the case of measures satisfying the FKG lattice property \cite{grimmett2006random}. However,
this property does not seem to hold obviously for random geometric graphs.
In the case of low-dimensional random geometric graphs (over the solid cube $[0,1]^d$), \cite{goel05monotoneproperties} show sharp-thresholds phenomena by proving that if $G_1, G_2$ are independent samples with densities $p(1-o(1)),p,$ then $G_1\subseteq G_2$ with high probability. The work of \cite{Bradonjic2013OnST} also deals with sharp thresholds on random geometric graphs, but again only applies to low dimensions. The methods of \cite{goel05monotoneproperties,Bradonjic2013OnST} do not seem applicable to the high-dimensional setting because both rely on the fact that a very fine (grid) subdivision of the space is well-covered by the latent vectors. In $d$ dimensions, the subdivision has $\exp(\Omega(d))$ cells, which is much larger than $n$ when $d = \omega(\log n).$
 
To the best of our knowledge, our result is the first to prove a generic sharp-thresholds statement for high-dimensional random geometric graphs in a non-trivial regime (i.e., when $\RGGsphere$ is not asymptotically the product distribution $\ergraph$ in total variation distance). 

\paragraph{Enumeration.} A classic result in algebraic geometry due to Warren \cite{warren1968lowerbounds} nearly immediately implies that the number of geometric graphs in $d$ dimensions is at most $(Cn/d)^{dn}$ for some explicit constant $C$ when $d = o(n)$ \cite{MCDIARMID2011627,SAUERMANN2021107593}. The main idea is that the edges of a geometric graph correspond to the sign patterns of $\binom{n}{2}$ polynomials over the $dn$ variables $\{(v_i)_j\}_{1\le i \le n, 1\le j \le d}.$ The variables are the coordinates of the latent vectors and the polynomials are the squared pairwise $\ell_2$ distance minus the radius squared.

Proving lower bounds, however, turns out to be a much more challenging task. In \cite{MCDIARMID2011627}, it is shown that in 2 dimensions the number of geometric graphs (known also as unit disk graphs in this case) is $n^{(2+o(1))n}.$ Using more sophisticated tools from algebraic geometry and topology, \cite{SAUERMANN2021107593} shows that the number of 
geometric graphs  in $d$ dimensions is $n^{(d+o(1))n}$ when $d = o(n).$

While our proof looses a non-trivial poly-logarithmic factor in the exponent, it is much simpler and relies on a simple probabilistic construction - spherical random geometric graphs.

\subsection{Organization}
In \cref{sec:preliminaries} we introduce some basic preliminaries and notation. In \cref{sec:nontechnical}, we give non-technical overviews of our two main algorithmic results: the coupling algorithm in \cref{thm:algorithmiccoupling} and the spectral refutation algorithm in \cref{thm:robustestingsos}. We give the full details in respectively \cref{sec:coupling} and \cref{sec:robusttesting}. In \cref{sec:enumeration} we prove \cref{thm:enumeration} via a rather simple counting argument using \cref{thm:algorithmiccoupling}. We end with several remarks and open questions regarding our results in \cref{sec:discussion}.




==> IntroductionV2.tex <==
% \section{Introduction}
% \begin{enumerate}
%     \item RGG is important: ``realistic" model (triangles etc.). RGG is mathematically interesting. Latent space graphs, Aldous-Hoover, old references on latent space graphs 1970, graphons. (The edge probabilities in social, biological, communication networks depend on features of the entities represented by nodes. Theoretical and empirical results show that geometric graphs fit well certain properties of brain networks \cite{vempala23kcap}, social networks \cite{Almagro22}, and protein-protein interaction networks \cite{higham08}.)
%     \item Define RGG -- MOST CANONICAL MODEL
%     \item The whole point of the model is that the edges are dependent. It turns out that for $d\gg (np)^3$, the model is conjectured to be close in TV to ER, therefore this is in some sense the completely uninteresting regime. When $\mathrm{\polylog}(n)\ll d \ll (np)^3$, very little is understood about the model. 
%     \item In low dimensions several striking phenomena.  HDX. 
%     \item Other properties such as spectral radius and clique number have various thresholds in $d$ that are far below the threshold for TV convergence. 
%     \item We ask to what extent do various characteristics and/or properties for ER hold for RGG? And for properties that RGG does have, can we determine the precise threshold in dimension? Where to start? In this paper we aim for general phenomena and graph properties.
%     \item One of the most fundamental features of ER graph is sharp threshold phenomenon for monotone graph properties. For RGG in quite low dimension, sharp thresholds. Completely mysterious in higher dimension. Even the connectivity threshold of RGG is not at all obvious. Similarly, not only the clique number, but counts of subgraphs (give some references as to why this is a big deal in combinatorics, rich literature).  
%     \item The question of whether RGG and ER are the same is TV. The question of whether RGG and ER are \emph{not too different} is Wasserstein. Just as TV is equivalent to \emph{hypothesis testing}, Wasserstein corresponds to a certain formulation of \emph{robust testing}. Model misspecification is an inevitability in statistical modeling and is needed to address the efficacy of real-world algorithms. 
    
%     % \item At high level, much of the work on high-dimensional random geometric graphs can be interpreted as comparing RGG to ER in some way. The interesting thing here is that there is a threshold dimension at which the model resembles or differs from ER. 
% \end{enumerate}

% \newpage
\section{Introduction}
% Random graphs have been a fundamental object of study since the seminal paper of Erd{\H o}s and R\'enyi \cite{Erdos1959ER}. In the \ERspace model $\ergraph,$ each edge among $n$ vertices appears independently with probability $p.$ More than 80 years of systematic study have revealed many marvels of the $\ergraph$ model. These have been instrumental to major developments in combinatorics, algorithm design and complexity, and network modeling. \emph{But what if we want to model dependence between edges? And why would we do so?} 

% \paragraph{1. Modeling Dependence via Random Geometric Graphs.}
Random geometric graphs have emerged as a fruitful way to model dependence between edges in random networks in both theory and practice \cite{penrose03}. Random geometric graphs capture the simple but omnipresent phenomenon that larger similarity in certain characteristics increases the likelihood of connection. This phenomenon is clearly illustrated by the canonical \emph{Spherical Random Geometric Graph}. 

\begin{definition}[Spherical Random Geometric Graph]
\label{def:sphericalrgg}
A sample from the distribution $\RGGsphere$ over graphs on $n$ vertices $[n] = \{1,\ldots, n\}$ of
dimension $d$ with expected density $p$ is generated as follows. First, $n$ vectors $V_1,  \ldots, V_n$ are drawn independently from the uniform distribution on the sphere $\dsphere.$ Then, an edge between $i$ and $j$ is formed if and only if $\langle V_i ,V_j\rangle \ge \tau^p_d.$ Here, $\tau^p_d$ is chosen so that $p = \prob[\langle V_i ,V_j\rangle \ge \tau^p_d].$ 
\end{definition}

In order to contextualize our results on the spherical model, we will first address the following question: 
\begin{center}\emph{What are the reasons to study random geometric graphs?}\end{center}
\begin{enumerate}
    \item \emph{Modeling Real-Life Networks:} 
    Random geometric graphs capture a type of dependence -- edge probabilities that depend on features of the entities represented by nodes -- which occurs in the real world and sciences. Theoretical and empirical results show that geometric graphs fit well certain properties of brain networks \cite{vempala23kcap}, social networks \cite{Almagro22}, and protein-protein interaction networks \cite{higham08}. \textbf{Remark:} We do not claim that any concrete generative model such as \cref{def:sphericalrgg} fits the data perfectly, even if it does so extremely well. This is an important point that we will return to!
\end{enumerate}
The theoretician may still wonder whether there are any benefits to studying random geometric graphs. In particular, \emph{what are the reasons to go beyond the classical $\ergraph$ model of Erd{\H o}s and R\'enyi, in which each edge between $n$ vertices appears {independently} with probability $p?$} 
\begin{enumerate}
    \item[2.]\emph{Understanding the Role of Independence in Combinatorial Phenomena:} $\ergraph$ exhibits a variety of deep phenomena, one of the prime examples being generic sharp-thresholds criteria for monotone properties \cite{Friedgut1999SharpTO}. \emph{Are such properties merely a virtue of the independence of edges or they also hold for other distributions?} In \cite{goel05monotoneproperties}, the authors address this question by showing that $n$-vertex random geometric graphs in dimension $d = o(\log n)$ exhibit sharp thresholds for monotone graph properties. 
    \item[3.]\emph{Combinatorial Constructions:} 
    While the importance of $\ergraph$ to combinatorial constructions cannot be overstated, starting with the application to Ramsey theory \cite{Erdos1959ER}, the model has limitations. For example, sparse \ERspace are provably not 2-dimensional expanders and a randomized construction for such was only given recently via \emph{random geometric graphs} in dimension $d = \Theta(\log n)$ \cite{Liu22Expander}. 
    \item[4.]\emph{Statistical Inference With Dependent Data:} Random geometric graphs provide a convenient model for developing tools for learning and estimation from dependent data. Lack of independence makes inference much more challenging but also more realistic due to the non-iid nature of real-life networks. A strikingly simple, but fundamental, question remains open after more than a decade of continuous work and improvements: 
    \emph{Can one even test for dependence, i.e. test between a random geometric graph and \ERspace}\cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}?    
\end{enumerate}

The answers to many of the aforementioned questions on random geometric graphs \emph{depend on the dimension}. Much of the early work (see \cite{penrose03} and references therein) on random geometric graphs focused on low dimensions $d = O(\log n)$ as well as the recent breakthrough on two-dimensional expanders \cite{Liu22Expander}. High-dimension was only considered much more recently, starting with \cite{Devroye11}. The majority of the existing work (\cite{Devroye11} being a notable exception) in this regime so far has focused on the following question: \emph{When is there dependence between the edges of $\RGGsphere?$} When $d\ll (np)^3,$ a simple triangle-based statistic witnesses edge dependence. Conjecturally, when $d\gg (np)^3,$ $\RGGsphere$ converges to $\ergraph$ in total variation distance. Yet, very little is known in the intermediate regime, which raises the question:   
\begin{center}
    \textit{Can we characterizes the dependence between edges of $\RGGsphere$ in the regime $\log(n)\ll d\ll (np)^3?$}
\end{center}
In the current work, we address this question with an eye towards the aforementioned reasons 1, 2, 3, and 4.
% , which is the focus of the majority of the existing works on \emph{high-dimensional} random geometric graphs thus far, is an important benchmark question. 
% Yet, it does not capture key aspects of the four directions outlined.

% In the current work, we also compare $\RGG$ and \ERspace but   Such a relaxation is motivated by all four reasons to study random geometric graphs that we outlined. 

% Understanding combinatorial phenomena in graphs with dependence between edges explicitly requires the distribution to \emph{not be} \ER. Statistical tasks in non-iid settings (beyond testing for independence) also require a distribution other than \ER. Finally, when modeling complex networks, it is too much to hope that all edges are explained by a simple generative model such as the one in \cref{def:sphericalrgg}. Even ignoring the simplicity of the threshold function $\indicator[\langle\cdot,\cdot\rangle\ge \tau^p_d],$ edges are only determined by pairwise compatibility of the feature vectors and higher-order effects are not captured. Additionally, in real-life networks, (potentially adversarial) corruptions might be present due to malicious entities or non-uniform errors in measurements. Again, testing in total variation is not the correct framework in the presence of corruptions. 

% For example, in social networks, the probability of a friendship may depend on a large variety of factors such as age, geographic location, education, occupation... \footnote{Even though, by no means we claim that any such set of factors fully determines whether there is a friendship. This is an important point that we will return to.} Correlations  

% Random graphs with underlying geometric structure are not only more realistic in modelling real-life networks, but also
% provide a fruitful counterpart to the well-studied \ER model for theoreticians. The dependence among edges leads to genuinely novel combinatorial phenomena (not shared by the simpler \ER model). At the same time, it also makes associated learning and estimation tasks in a non-iid setting much more challenging (but also more realistic due to the non-iid nature of real-life networks).



% Random geometric graphs in low dimension have been extensively studied (see \cite{penrose03} and references therein). The study of the high-dimensional regime in which $d$ grows with $n,$ potentially even at a polynomial rate, however, was more recently initiated by 
% \cite{Devroye11}. In \cite{Devroye11}, the authors discuss both \emph{combinatorial properties} of the distribution, concretely the typical size of the largest clique, as well as \emph{statistical tasks}, namely testing between a random geometric graph and \ER with a single sample. Since then, both directions have flourished. . Determining the regime in which the testing problem is information theoretically possible is still open even though it has witnessed continuous progress  Other statistical tasks have also been studied such as dimension estimation \cite{Bubeck14RGG} and recovering the latent vectors from the graph data \cite{li2023spectral}.  

\subsection{Our Contributions} 
\subsubsection{Our Angle}
We will aim for a characterization of random geometric graphs that allows us to address two previously unexplored themes in the $\log (n)\ll d \ll (np)^3$ regime: \emph{sharp thresholds for edge-monotone properties} and \emph{robustness to bounded edge corruptions.} The combination of \emph{monotonicity} and \emph{edge corruptions} leads us to the following \emph{approximate stochastic dominance} comparison with \ERspace (see also \cite{Liu2022STOC}):
\begin{equation}
\label{eq:couplinquestion}
\tag{Q1}
\begin{split}
    &\textit{When can one couple the two graph distributions in such a way that with high probability}\\
    &\quad\quad\quad\quad\quad\mathsf{G}(n,p(1-\epsilon))\subseteq \RGGsphere \subseteq\mathsf{G}(n,p(1+\epsilon))\textit{ for some small } \epsilon?
    \end{split}
\end{equation}
Here, inclusion is over the edge set. Our main result
is that such a coupling exists if and only if $d\gg np.$ Exploiting this fact, we address aspects of all four of the aforementioned directions:
\begin{enumerate}
    \item \emph{Modeling Real-Life Networks:} Random geometric graphs with few (but otherwise arbitrary) edge corruptions more accurately model real-life networks due to the potential presence of edges not explained by the geometry. These could be due to model misspecifications (it is perhaps too much to hope that all edges are explained by a simple generative model such as the one in \cref{def:sphericalrgg}) or corruptions in the observations due to adversarial interference and measurement errors.
    \item \emph{Understanding the Role of Independence in Combinatorial Phenomena:} We use the \emph{edge-monotonicity} of the coupling to compare monotone properties of $\ergraph$ and $\RGGsphere.$ We give the first proof of sharp thresholds for monotone properties of $\RGG$ in a non-trivial high-dimensional regime.
    \item \emph{Combinatorial Constructions:} A coupling of the form in \cref{eq:couplinquestion} implies a lower bound on the support size of the $\RGGsphere$ distribution. This allows us to use $\RGGsphere$ as a randomized construction for 
    counting the number of geometric graphs in dimension $d.$ 
    \item \emph{Statistical Inference With Dependent Data:} One interpretation of the approximate stochastic dominance is that a sample of $\ergraph$ is a sample of $\RGGsphere$ with $O(\epsilon n^2 p)$ adversarially corrupted edges. This leads us to consider the well-studied question of testing between $\ergraph$ and $\RGGsphere$ \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier} in the previously unexplored setting of adversarial edge-corruptions.  
\end{enumerate}

\subsubsection{Characterizing Edge Dependence in RGG: Main Theorem and Interpretation}
% Motivated by the last consideration -- model mis-specifications and adversarial corruptions -- we choose to study a comparison which allows for a fraction of unexplained edges. Our main theorem is the following algorithmic result.

\begin{theorem}[Main Coupling Result]
\label{thm:algorithmiccoupling}
Consider some $n,d,p$ such that $d= \Omega( \max(np,\log n))$ and $p = \Omega(1/n), p\le 1/2.$ There exists a polynomial-time algorithm which on input $H\sim \ergraph,$ outputs $n$ vectors $V_1 = V_1(H), V_2 = V_2(H), \ldots, V_n = V_n(H)$ in $\dsphere$ with the following two properties:
\begin{enumerate}
    \item The marginal distribution of the vectors is independent uniform: $V_1, V_2, \ldots, V_n\iidsim\unif(\dsphere).$
    \item With high probability (over the input and internal randomness), $\indicator[\langle V_i, V_j\rangle\ge \tau^p_d] = H_{ij}$ for all pairs $i,j$ such that $|\langle V_i, V_j\rangle - \tau_p^d|\ge \frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{3/2}}{d}$ for some absolute constant $c.$
     
\end{enumerate}
\end{theorem}
In other words, the algorithm described above couples $\RGG$ and $\ergraph$ in such a way that they only differ at pairs $(i,j)$ for which $\langle V_i, V_j\rangle $ is very close to the threshold. Elementary calculations shows that with high probability, $G,H$ differ at only $\tilde{O}\Big(\binom{n}{2}p\times\sqrt{\frac{{np}}{d}}\Big) = o\Big(\binom{n}{2}p\Big)$ edges. An immediate implication of \cref{thm:algorithmiccoupling} is the following approximate  stochastic dominance. 

\begin{corollary}[Approximate Stochastic Dominance]
\label{thm:stochasticcoupling}
Consider some $n,d,p$ such that $d= \Omega(np\log^4 n, \log^5n)$ and $p = \Omega(1/n).$ Then, there exists a coupling of $G\sim\RGG(n,\dsphere,p),$ $H_-\sim \mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ and $ H_+\sim \mathsf{G}(n,p(1+\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})),$ 
 such that 
$
H_-\subseteq G \subseteq H_+
$
with high-probability, where inclusion is defined as inclusion over the edge set.
\end{corollary}

In \cite{Liu2022STOC}, the authors prove \cref{thm:stochasticcoupling} under the weaker condition $d \ge \polylog(n)\times n^2p^2$ with the purpose of describing the local structure of random geometric graphs. Our stronger result, based on an entirely different proof technique, is crucial for some of the applications to follow.

Note that $d =\tilde{\Theta}(np)$ is a polynomially smaller dimension than the one required for\linebreak $\TV(\RGGsphere, \ergraph) = o(1),$ For the latter statement to hold, $d= \tilde{\Omega}(n^3p^3)$ is needed as demonstrated by the signed triangle count test \cite{Bubeck14RGG,Liu2022STOC} which is also conjectured to be optimal \cite{Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}. While $d = \tilde{\Theta}(n^3p^3)$ is still rather mysterious, the critical dimension in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} $d = \tilde{\Theta}(np)$ has two natural coalescent interpretations:
\begin{enumerate}
    \item \textbf{Entropic Threshold:} The maximal entropy of a graph with expected density $p$ is $\binom{n}{2}H(p) = \tilde{\Theta}(n^2p)$ and this is achieved by $\ergraph.$ On the other hand, the following heuristic (which we make rigorous in \cref{sec:enumeration}) suggests that the entropy of $\RGGsphere$ is at most $\tilde{\Theta}(nd).$  $\dsphere$ has an $\epsilon$-net of size $\exp(\tilde{O}(d\log(1/\epsilon))).$ 
    Hence, we can discretize the sphere into $\exp(\tilde{O}(d))$ points. As there are $n$ latent vectors $V_1, V_2, \ldots, V_n,$ each effectively of the $\exp(\tilde{O}(d))$-discretization, and the latent vectors uniquely determine the geometric graph, the $\RGGsphere$ distribution effectively has support size 
    $\exp(\tilde{O}(nd)).$ Hence, its entropy is at most $\tilde{O}(nd).$ To match (up to lower order terms) the $\tilde{\Theta}(n^2p)$ entropy of $\ergraph,$ one therefore needs $d = \tilde{\Omega}(np).$ Using \cref{thm:algorithmiccoupling}, in \cref{sec:enumeration} we show that when $d = \tilde{\Omega}(np),$ the support size of $\RGGsphere$ is indeed ``maximal'', i.e. of size $\exp(\tilde{\Omega}(n^2p)).$
    \item \textbf{Spectral Threshold:} Miraculously, as soon as $d \lesssim np,$ there is a spectral separation between $\ergraph$ and $\RGGsphere.$ 
    The second largest eigenvalue of $\ergraph$ is $\tilde{\Theta}(\sqrt{np})$ while the second largest eigenvalue of $\RGGsphere$ is 
    $\tilde{\Theta}({\frac{np}{\sqrt{d}}})\gg \tilde{\Theta}(\sqrt{np})$
    \cite{Liu22Expander,li2023spectral}.
    This spectral separation allows for efficient spectral and SDP algorithms, as in \cite{li2023spectral} and \cref{sec:robusttesting}.
\end{enumerate}

% We will get back to this point in \cref{sec:discussion}, but we believe that the coincidence of entropic and spectral thresholds for the $\RGGsphere$ distributions heuristically explains why no information-computation gaps have been observed for natural statistical tasks such as testing, robust testing, and embedding of random geometric graphs. As soon as there is a very strong information theoretic separation between $\RGG$ and $\ergraph,$ there is also a computationally efficient (spectral) witness.

\begin{remark} We note that in general a relaxed stochastic dominance of the form in \cref{thm:stochasticcoupling} does not guarantee closeness in total variation even if one couples 
$H_-\sim \mathsf{G}(n,p), H_+\sim \mathsf{G}(n,p), G\sim\mathcal{D}$ such that $H_-\subseteq G\subseteq H_+$ with high probability for some $\mathcal{D}.$ Specifically, consider a distribution $\mathcal{D}$ defined by the following coupling. $H_-$ is drawn from $\ergraph.$ Then, $H_+$ is a copy of $H_-$ except that a uniformly random non-edge is changed to an edge. One can check that whenever $p= \Omega(1/n),$ the distribution of $H_+$ is only $o(1)$ TV distance away from $\ergraph.$ Finally, $G$ is the graph among $H_-, H_+$ with an even number of edges. Clearly, $H_-\subseteq G\subseteq H_+$  w.h.p. but $\TV(\mathcal{D}, \ergraph) \ge 1/2 - o(1)$ as the distribution $\mathcal{D}$ is supported on graphs with an even number of edges.
\end{remark}
\subsubsection{Understanding the Role of Independence: Sharp Thresholds} The coupling in \cref{thm:stochasticcoupling} between random geometric graphs and \ERspace is monotone in the sense that 
$
H_-\subseteq G \subseteq H_+.
$
Whenever $H_-\sim \mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ satisfies an increasing property with high probability, so does $G\sim \RGGsphere.$ Whenever 
$G\sim \RGGsphere$ satisfies an increasing property, so does $H_+\sim \mathsf{G}(n,p(1+\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})).$ 
This immediately allows us to translate sharp-threshold phenomena from \ERspace to RGG by considering the couplings between $G_-\subseteq H_-$ 
where 
$G_-\sim \RGG(n,\dsphere,p(1-3\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ and  
$H_+\subseteq G_+ $ where
$G_+\sim \RGG(n,\dsphere,p(1+3\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})).$

\begin{theorem} Suppose that $\mathcal{P}_n$ is a monotone property with critical probability $p^c_n$ which satisfies $p^c_n = \Omega(1/n).$ 
Suppose further that $\mathcal{P}_n$ exhibits a sharp threshold with respect to $\ergraph$ and has a critical window of length $\omega_\epsilon = o(p^c_n).$ 
If $d_n=  \omega(\max(np^c_n\log^4 n, \log^5n)),$ the property $\mathcal{P}_n$ also exhibits a sharp threshold with respect to $\RGG(n,d_n,p)$ and has critical probability $p^c_n + O\Big(p_n^c\frac{\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}\Big)$ and critical window of length 
$\omega_\epsilon  +  O\Big(p_n^c\frac{\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}\Big).$
\end{theorem}

This theorem partially answers in the affirmative a question due to Perkins on whether high-dimensional random geometric graphs exhibit sharp thresholds \cite{perkins2024searching}. 
\subsubsection{Combinatorial Constructions: Enumeration}  \cref{thm:stochasticcoupling} demonstrates that $\RGGsphere$ is a distribution over at least $\exp(\tilde{\Omega}(n^2p))$ graphs when $d= \max(np\log^4 n, \log^5 n).$ The proof is rather simple - if $\mathcal{M}$ is the support of $\RGGsphere,$ using a simple counting argument one can bound the number of graphs that are edge-subgraphs of some graph $H$ in $\mathcal{M}$ and differ from $H$ in $o(\binom{n}{2}p)$ edges. Using this bound, one can arrive at an upper bound for the entropy of $\mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ (which is $\tilde{\Theta}(n^2p)$).  This, in turn, implies a lower bound on $|\mathcal{M}|.$ Altogether, this gives the following result.

\begin{theorem}
\label{thm:enumeration}
The number of graphs which can be realized as intersection graphs of unit spheres in dimension $d$ is at least $\exp(nd\log^{-7}n).$     
\end{theorem}

The statement is tight up to the $\log$ terms as shown in \cite{SAUERMANN2021107593}. The result is not new and sharper estimates (up to the log terms) were recently shown in \cite{SAUERMANN2021107593}. Nevertheless, one advantage of our proof is its simplicity - it is based on a natural probabilistic construction, spherical random geometric graphs. The techniques from algebraic geometry and algebraic topology in \cite{SAUERMANN2021107593} are significantly more involved, even though admittedly much more systematic and sharper.

\subsubsection{Inference with Dependent Data: Robust Testing} One immediate application of \cref{thm:stochasticcoupling} is  the following. Suppose that 
$\epsilon\in (0,1]$ is a small fixed constant. Whenever $d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5)$ (where $K(\epsilon)$ depends solely on $\epsilon$), one can with high probability (adversarially) corrupt $\epsilon \binom{n}{2}p$ edges of a sample from $\RGGsphere$ and produce a sample from $\ergraph.$
Hence, the following robust testing problem is information-theoretically impossible when $d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5):$ 
\begin{problem}[Robust Testing of Geometry With Edge Corruptions]
\label{problem:robusttesting}
Given are $n,d\in \mathbb{N},$ $p\in [0,1]$ and a fixed constant $\epsilon.$
Consider the following hypothesis testing problem. One observes a graph $H$ and needs to decide between $H_0: H = \mathcal{A}(\bfG),\bfG\sim \ergraph$ and 
$H_1: H = \mathcal{A}(\bfG),\bfG\sim \mathsf{RGG}(n,d,p).$ Here $\mathcal{A}$ is an arbitrary adversary who is allowed to corrupt at most $\epsilon \binom{n}{2}p$ edges and non-edges.
\end{problem}
We restrict the adversary to changing $\epsilon \binom{n}{2}p$ edges for a small constant $\epsilon$ as the robust testing problem is otherwise trivially impossible. Both $\mathsf{RGG}(n,d,p)$ and 
$\ergraph$ have with high probability $1.5\binom{n}{2}p$ edges. Hence, an adversary $
\mathcal{A}$ who simply deletes all edges of a sample from $\RGG$ and then inserts Bernoulli $p$ edges (in total $3\binom{n}{2}p$ w.h.p.) can transform into a sample from $\ergraph.$ Thus, \cref{problem:robusttesting} captures the setting of ``maximal adversaries.'' 

\begin{remark}[Efficient adversaries]
\label{rmk:eficientadversary}
When $d = o((np)^3(\log n)^3), d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5)),$ \cref{problem:robusttesting} is information theoretically impossible even against polynomial-time adversaries. In this regime, an adversary can see a sample $H$ and (correctly with high probability) test using the signed-triangle statistic \cite{Liu2022STOC} whether the sample is from $\ergraph$ or $\RGGsphere.$ If $H$ is from $\ergraph,$ the adversary can use the efficient algorithm from \cref{thm:algorithmiccoupling} and produce (with high-probability) a sample from $\RGGsphere$ differing from $H$ only at $o\Big(\binom{n}{2}p\Big)$ edges. If $H$ is from $\RGG$ already, the adversary does not change edges. 
\end{remark}



Due to the miraculous coincidence of spectral and entropic thresholds, \cref{problem:robusttesting} is solvable in polynomial time even against computationally unbounded adversaries when $d\ll np.$ 

\begin{theorem}
\label{thm:robustestingsos}
There exists some constant absolute constant $K_r>0$ with the following property. When $d\le K_r\min(np\log(1/p), n^2p^2\log(1/p)\log^{-2}n)$ and $d = \omega(\log 1/p),$ there exists a polynomial-time algorithm solving \cref{problem:robusttesting} with high probability for all $\epsilon\le K_r.$
\end{theorem}
We overview the algorithm in \cref{sec:nontechnicalrobust} and give full detail in \cref{sec:robusttesting}. It is a constant degree SoS program for spectral refutation of a small operator norm of the centered adjacency matrix. The key insight, implicit in \cite{li2023spectral}, is that the latent vectors witness a large second eigenvalue for a random geometric graph. The approach works for robust testing against any null hypothesis with a substantially smaller second eigenvalue than $\RGGsphere,$ see \cref{rmk:testingrobustly}.

\begin{remark}
\label{rmk:couplingimpossibilityfromspectral}
\cref{thm:robustestingsos} implies that when $d \le K_r\min(np\log(1/p), n^2p^2\log(1/p)\log^{-2}n),$ there does not exist a coupling between $H_-\sim \mathsf{G}(n,p(1-o(1)),G\sim \RGGsphere, H_+\sim \mathsf{G}(n,p(1+o(1))$
such that $H_-\subseteq G\subseteq H_+$ w.h.p. Otherwise, one can use this coupling as an adversary for \cref{problem:robusttesting} even against computationally-unbounded testers but \cref{thm:robustestingsos} shows that such an adversary cannot exist. Hence, the dimension requirement $d = \tilde{\Omega}(np)$ in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} is tight (up to $\polylog$ factors).
\end{remark}



\subsection{Prior Work and Challenges}
\paragraph{Coupling Random Geometric Graphs and \ER.} In \cite{Liu2022STOC}, the authors prove \cref{thm:stochasticcoupling} under the weaker condition $d\ge n^2p^2\log^4n.$ In their construction, they sample $V_1, V_2, \ldots, V_n$ sequentially. A caricature of their argument is that with high probability, when sampling $V_1, V_2, \ldots, V_{k-1}$ the intersection of any $i\approx pk$ $p$-caps and $k-i-1\approx k(1-p)$ $p$-anti-caps corresponding to $V_1, V_2, \ldots, V_{i-1}$\footnote{For $V\in \dsphere,$ the associated $p$-cap is the set $\{U \in \dsphere\; : \langle U, V\rangle\ge \tau^p_d\}$  and the $p$-anti-cap is its complement} is sufficiently close to $p^{i}(1-p)^{k-i-1}.$ Hence, one should expect that the edges from $k$ to $[k-1]$ roughly are distributed as ``independent'' $\Bernoulli(p)$ variables. They make this statement precise by quantifying ``sufficiently close'' via a concentration argument based on transportation inequalities. While our proof of \cref{thm:stochasticcoupling} is entirely different, it suggests what might be suboptimal in the approach of \cite{Liu2022STOC}. Typical intersections of $\approx pk$ caps and $k-i-1\approx k(1-p)$ anti-caps might concentrate much better than worst-case 
intersections due to a square-root cancellation phenomenon. We use this idea in our proof to get $d\ge \max(np, \log n)$ and if we consider \emph{all} intersections of caps and anti-caps instead, we also obtain a result for $d\ge n^2p^2\polylog n.$ While the square-root cancellation comes naturally in our martingale-based analysis, it is unclear whether it can be incorporated in the transportation-based approach of \cite{Liu2022STOC}. Even beyond that, an advantage of our approach is that there is an efficient algorithm producing the coupling -- \cref{thm:algorithmiccoupling}. The result of \cite{Liu2022STOC} is not obviously algorithmically efficient as it requires keeping track of an intersection of caps and anti-caps on the sphere and being able to sample and estimate the volume of this intersection.    

A different work which shows that in certain regimes random geometric graphs can be represented as $\ergraph$ with some planted structure (i.e. the edges on locations for which $|\langle V_i, V_j\rangle - \tau_p^d|\le \frac{\sqrt{np\log n}}{d}$ in \cref{thm:algorithmiccoupling}) is 
\cite{bangachev2024fourier}. In fact, in their representation, again the non-\ERspace pairs $(i,j)$ are exactly the ones for which $\langle V_i, V_j\rangle$ are close to $\tau^p_d$ (called \emph{fragile pairs} in \cite{bangachev2024fourier}). While some of our ideas are related to and motivated by \cite{bangachev2024fourier}, there is a fundamental barrier to their proof technique. It crucially relies on performing the Gram-Schmidt operation on the latent vectors\footnote{To be fully precise, the Gram-Schmidt is performed on the isotropic Gaussian vectors $Z_1, Z_2, \ldots, Z_n.$ 
% where $Z_i = V_i \chi_i$ (where $\chi_i$ is an appropriate square root of a $\chi^2$ random variable). 
This, however, makes little difference to the arguments in \cite{bangachev2024fourier} and the current work, see \cref{rmk:sphericaltogaussian}.} $V_1, V_2, \ldots, V_n.$ In particular, this method requires $d\ge n,$ so obtaining a result of the form in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} for $d\ll n$ is impossible. 

\paragraph{Testing.} To the best of our knowledge, this work is the first to study the robust testing problem between $\RGGsphere$ and \ER. The same question in the setting of no edge corruptions has attracted significant attention in recent years \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}. Formally, one observes a graph $G$ and needs to decide $H_0:G\sim \ergraph$ or $H_1:G\sim \RGGsphere.$ By counting signed triangles, i.e computing $\sum_{i<j<k}(G_{ij} - p)(G_{jk}-p)(G_{ki}-p),$ one can succeed with high probability whenever $d = \omega(n^3p^3\log^3(1/p))$ \cite{Bubeck14RGG,Schramm_2022}.  The current state-of-the-art information-theoretic lower bounds are that when $d\ge (\log n)^C n^3p^2,$ the problem is information theoretically impossible as well as when 
$p = \Theta(1/n)$ and $d\ge (\log n)^C$ for some constant $C$ \cite{Liu2022STOC}. Even ignoring $\polylog $ factors, there is still a $1/p$ gap between the testing algorithm and the information-theoretic lower bound when $1/n\ll p\ll 1/2.$ The gap was recently closed with respect to low-degree polynomial tests by \cite{bangachev2024fourier}: counting signed triangles is optimal among all degree $\log^{2-\epsilon} n$ polynomial tests.

We note that both the question of upper and lower-bounds are significantly different when one considers the testing problem with a constant number of adversarial corruptions as in \cref{problem:robusttesting}. On the algorithmic side, simple counting tests such as counting signed triangles necessarily fail. For example, the expected number of signed triangles in $\RGGsphere$ is $\tilde{\Theta}(n^3p^3/\sqrt{d})$ \cite{Liu2022STOC}. One can increase the expected number of signed triangles in $\ergraph$ by planting a clique of size $\tilde{O}(np/d^{1/6})$ which requires $\tilde{O}(n^2p^2/d^{1/3}) = o(n^2p)$ adversarial corruptions. One can argue similarly for other subgraph-counting tests. This is why we need a more sophisticated sum-of-squares spectral refutation algorithm which uses the true embedding as a witness. To the best of our knowledge, \cite{mao2024informationtheoretic} is the only other work which uses an embedding-based approach for testing for random geometric graphs, but their work is in low-dimension and the algorithm is not computationally efficient. Regarding lower-bounds, all of the prior work on the setting without adversarial corruptions \cite{Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC} very strongly exploits distributional assumptions (such as the relationship to Wishart ensembles and a certain $\KL$-convexity argument revealing the latent vectors). We do not expect that any of these techniques applies to the adversarial setting. Instead, we rely on our coupling argument \cref{thm:stochasticcoupling}.

Finally, there is still a gap between the known upper-bound $\tilde{\Theta}(n^3p^3)$ and the lower-bound $\Tilde{\Theta}(n^3p^2)$ in the setting of no corruptions when $p = \omega(1/n).$ In this work, we determine that (up to log factors) $d = \Tilde{\Theta}(np)$ is the tight threshold for testing with adversarial corruptions computationally and information-theoretically. Part of the reason for this difference between the robust setting and the setting without corruptions is how well we understand the respective thresholds. $d = \Tilde{\Theta}(np)$ has a very clear significance - as an entropic threshold information-theoretically and as a spectral threshold computationally. Yet, the condition $d = \Tilde{\Theta}(n^3p^3)$ so far seems to only have a computational interpretation. It is the threshold below which one can test counting signed triangles, which are ``the most informative subgraph'' among $\log^{2-\epsilon}n$-sized subgraphs \cite{bangachev2024fourier}. The search for the correct information-theoretic interpretation of  $d = \Tilde{\Theta}(n^3p^3)$ remains open.

\paragraph{Sharp Thresholds.} The question of whether monotone properties exhibit sharp thresholds is by far the best understood in the case of product distributions. The seminal paper of \cite{Friedgut1999SharpTO} establishes very broad conditions on vertex-transitive properties for which the \ERspace distribution exhibits sharp-thresholds. In non-product settings, much less is understood. Important progress has been made in the case of measures satisfying the FKG lattice property \cite{grimmett2006random}. However,
this property does not seem to hold obviously for random geometric graphs.
In the case of low-dimensional random geometric graphs (over the solid cube $[0,1]^d$), \cite{goel05monotoneproperties} show sharp-thresholds phenomena by proving that if $G_1, G_2$ are independent samples with densities $p(1-o(1)),p,$ then $G_1\subseteq G_2$ with high probability. The work of \cite{Bradonjic2013OnST} also deals with sharp thresholds on random geometric graphs, but again only applies to low dimensions. The methods of \cite{goel05monotoneproperties,Bradonjic2013OnST} do not seem applicable to the high-dimensional setting because both rely on the fact that a very fine (grid) subdivision of the space is well-covered by the latent vectors. In $d$ dimensions, the subdivision has $\exp(\Omega(d))$ cells, which is much larger than $n$ when $d = \omega(\log n).$
 
To the best of our knowledge, our result is the first to prove a generic sharp-thresholds statement for high-dimensional random geometric graphs in a non-trivial regime (i.e., when $\RGGsphere$ is not asymptotically the product distribution $\ergraph$ in total variation distance). 

\paragraph{Enumeration.} A classic result in algebraic geometry due to Warren \cite{warren1968lowerbounds} nearly immediately implies that the number of geometric graphs in $d$ dimensions is at most $(Cn/d)^{dn}$ for some explicit constant $C$ when $d = o(n)$ \cite{MCDIARMID2011627,SAUERMANN2021107593}. The main idea is that the edges of a geometric graph correspond to the sign patterns of $\binom{n}{2}$ polynomials over the $dn$ variables $\{(v_i)_j\}_{1\le i \le n, 1\le j \le d}.$ The variables are the coordinates of the latent vectors and the polynomials are the squared pairwise $\ell_2$ distance minus the radius squared.

Proving lower bounds, however, turns out to be a much more challenging task. In \cite{MCDIARMID2011627}, it is shown that in 2 dimensions the number of geometric graphs (known also as unit disk graphs in this case) is $n^{(2+o(1))n}.$ Using more sophisticated tools from algebraic geometry and topology, \cite{SAUERMANN2021107593} shows that the number of 
geometric graphs  in $d$ dimensions is $n^{(d+o(1))n}$ when $d = o(n).$

While our proof loses a non-trivial poly-logarithmic factor in the exponent, it is much simpler and relies on a simple probabilistic construction - spherical random geometric graphs.

\paragraph{Other Works on Random Geometric Graphs in The Regime $\log(n)\ll d\ll (np)^3.$} In \cite{Devroye11}, the authors show that as long as $d\gg \polylog(n), $ the clique numbers of $\ergraph$ and $\RGGsphere$ are essentially the same. While their work is also focused on a comparison with \ERspace in a metric other than total variation distance, one major difference is that it is only for a single (monotone) property, the clique number. Our coupling result addresses \emph{all} monotone properties.   

\subsection{Organization}
In \cref{sec:preliminaries} we introduce some basic preliminaries and notation. In \cref{sec:nontechnical}, we give non-technical overviews of our two main algorithmic results: the coupling algorithm in \cref{thm:algorithmiccoupling} and the spectral refutation algorithm in \cref{thm:robustestingsos}. We give the full details in respectively \cref{sec:coupling} and \cref{sec:robusttesting}. In \cref{sec:enumeration} we prove \cref{thm:enumeration} via a rather simple counting argument using \cref{thm:algorithmiccoupling}. We end with several remarks and open questions regarding our results in \cref{sec:discussion}.




==> IntroductionV3.tex <==
% \section{Introduction}
% \begin{enumerate}
%     \item RGG is important: ``realistic" model (triangles etc.). RGG is mathematically interesting. Latent space graphs, Aldous-Hoover, old references on latent space graphs 1970, graphons. (The edge probabilities in social, biological, communication networks depend on features of the entities represented by nodes. Theoretical and empirical results show that geometric graphs fit well certain properties of brain networks \cite{vempala23kcap}, social networks \cite{Almagro22}, and protein-protein interaction networks \cite{higham08}.)
%     \item Define RGG -- MOST CANONICAL MODEL
%     \item The whole point of the model is that the edges are dependent. It turns out that for $d\gg (np)^3$, the model is conjectured to be close in TV to ER, therefore this is in some sense the completely uninteresting regime. When $\mathrm{\polylog}(n)\ll d \ll (np)^3$, very little is understood about the model. 
%     \item In low dimensions several striking phenomena.  HDX. 
%     \item Other properties such as spectral radius and clique number have various thresholds in $d$ that are far below the threshold for TV convergence. 
%     \item We ask to what extent do various characteristics and/or properties for ER hold for RGG? And for properties that RGG does have, can we determine the precise threshold in dimension? Where to start? In this paper we aim for general phenomena and graph properties.
%     \item One of the most fundamental features of ER graph is sharp threshold phenomenon for monotone graph properties. For RGG in quite low dimension, sharp thresholds. Completely mysterious in higher dimension. Even the connectivity threshold of RGG is not at all obvious. Similarly, not only the clique number, but counts of subgraphs (give some references as to why this is a big deal in combinatorics, rich literature).  
%     \item The question of whether RGG and ER are the same is TV. The question of whether RGG and ER are \emph{not too different} is Wasserstein. Just as TV is equivalent to \emph{hypothesis testing}, Wasserstein corresponds to a certain formulation of \emph{robust testing}. Model misspecification is an inevitability in statistical modeling and is needed to address the efficacy of real-world algorithms. 
    
%     % \item At high level, much of the work on high-dimensional random geometric graphs can be interpreted as comparing RGG to ER in some way. The interesting thing here is that there is a threshold dimension at which the model resembles or differs from ER. 
% \end{enumerate}

% \newpage
\section{Introduction}
% Random graphs have been a fundamental object of study since the seminal paper of Erd{\H o}s and R\'enyi \cite{Erdos1959ER}. In the \ERspace model $\ergraph,$ each edge among $n$ vertices appears independently with probability $p.$ More than 80 years of systematic study have revealed many marvels of the $\ergraph$ model. These have been instrumental to major developments in combinatorics, algorithm design and complexity, and network modeling. \emph{But what if we want to model dependence between edges? And why would we do so?} 

% \paragraph{1. Modeling Dependence via Random Geometric Graphs.}
Random geometric graphs have emerged as a fruitful way to model dependence between edges in random networks in both theory and practice \cite{penrose03}. Random geometric graphs capture the simple but omnipresent phenomenon that larger similarity in certain characteristics increases the likelihood of connection.   Random geometric graphs capture a type of dependence -- edge probabilities that depend on features of the entities represented by nodes -- which occurs in the real world and sciences. Theoretical and empirical results show that geometric graphs fit well certain properties of brain networks \cite{vempala23kcap}, social networks \cite{Almagro22}, and protein-protein interaction networks \cite{higham08}. 
% \textbf{Remark:} We do not claim that any concrete generative model such as \cref{def:sphericalrgg} fits the data perfectly, even if it does so extremely well. 
\cite{mcfarland1973social,mcpherson2001birds,hoff2002latent}. 

Perhaps the most canonical instance is the \emph{Spherical Random Geometric Graph}. 

\begin{definition}[Spherical Random Geometric Graph]
\label{def:sphericalrgg}
A sample from the distribution $\RGGsphere$ over graphs on $n$ vertices $[n] = \{1,\ldots, n\}$ of
dimension $d$ with expected density $p$ is generated as follows. First, $n$ vectors $V_1,  \ldots, V_n$ are drawn independently from the uniform distribution on the sphere $\dsphere.$ Then, an edge between $i$ and $j$ is formed if and only if $\langle V_i ,V_j\rangle \ge \tau^p_d.$ Here, $\tau^p_d$ is chosen so that $p = \prob[\langle V_i ,V_j\rangle \ge \tau^p_d].$ 
\end{definition}

Much of the work on the high-dimensional RGG 
can be interpreted as comparison to \ER, with the dimension $d$ determining to what extent the underlying geometry impacts the resulting graph. At one extreme, if $d$ is sufficiently large, the RGG distribution approaches \ERspace in total variation.
% As the dimension $d$ grows relative to the number of nodes $n$, it turns out that the model becomes close in total variation to \ER. 
The problem of determining the threshold in $d$ where total variation convergence occurs, as both $n$ and $d$ grow large, has attracted significant attention in recent years \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}, with steady progress towards proving the conjectured threshold $d\gg (np)^3 \log^3(1/p)$. 
% Formally, one observes a graph $G$ and needs to decide $H_0:G\sim \ergraph$ or $H_1:G\sim \RGGsphere.$ By counting signed triangles, i.e computing $\sum_{i<j<k}(G_{ij} - p)(G_{jk}-p)(G_{ki}-p),$ one can succeed with high probability whenever $d = \omega(n^3p^3\log^3(1/p))$ \cite{Bubeck14RGG,Schramm_2022}.  The current state-of-the-art information-theoretic lower bounds are that when $d\ge (\log n)^C n^3p^2,$ the problem is information theoretically impossible as well as when 
% $p = \Theta(1/n)$ and $d\ge (\log n)^C$ for some constant $C$ \cite{Liu2022STOC}. Even ignoring $\polylog $ factors, there is still a $1/p$ gap between the testing algorithm and the information-theoretic lower bound when $1/n\ll p\ll 1/2.$ The gap was recently closed with respect to low-degree polynomial tests by \cite{bangachev2024fourier}: counting signed triangles is optimal among all degree $\log^{2-\epsilon} n$ polynomial tests.
When the RGG is close in total variation to \ER, the models are information-theoretically indistinguishable; in this regime the latent geometry plays no role and the RGG is uninteresting. 

The complementary regime $d\ll (np)^3$, where the RGG exhibits meaningful dependencies between edges, is the one of interest both in capturing features of real-world graphs and from the mathematical side. In this regime the signed triangle statistic \cite{Bubeck14RGG} successfully distinguishes the two models. But this is \emph{just one particular way} of measuring similarity of the two models. What about other properties? It turns out that RGG and \ERspace are similar in some regards and different in others. 
As a recent fascinating demonstration of how dependence in RGG makes it quite different from \ER, \cite{Liu22Expander} showed that in dimension $d = \Theta(\log n)$ 
RGGs are
2-dimensional expanders. 
Other properties, such as the size of the maximum clique \cite{Devroye11}, are almost the same as soon as ???. \gb{mention spectral difference for $d\ll np$}
% At the same time, the \ERspace graph has a vast literature and is by now well-understood, so it would be nice to leverage this towards a better understanding of RGG. 

% For RGGs in dimension $d$ where the model is very different from \ER, can we nevertheless show that certain basic phenomena appearing in \ERspace also appear in RGG? 

% Notions of comparison between RGG and \ERspace other than total variation 


A rather deep fact about the \ERspace graph $\ergraph$ is that \emph{all monotone properties} exhibit a sharp-threshold in $p$ \cite{Friedgut1999SharpTO}. 
In non-product settings, much less is understood. Important progress has been made in the case of measures satisfying the FKG lattice property \cite{grimmett2006random}, however, the RGG does not satisfy this property. Does the sharp threshold phenomenon hold also for RGG?
In \cite{goel05monotoneproperties}, the authors answer this question affirmatively in \emph{low dimension} $d = o(\log n)$. One of the main applications of our results is to show that sharp thresholds hold also in RGG in moderately high dimension $d\gg ???$. \gb{and at same location?} We remark that aside from existence of a clique of a given size, as studied in \cite{Devroye11}, even determining the threshold for connectivity, Hamiltonicity, or virtually any other monotone property for RGG was open. 

Returning to comparison of RGG and \ER, total variation captures the most basic notion of comparison: given a graph sampled from one of two distributions, can we guess which one?
Large total variation between the two distributions for $d\ll (np)^3$ implies the existence of \emph{some} test, but as we will show, all tests for $d\gg np$ are extremely brittle. 

One way to make precise the aim of elucidating meaningful differences between two distributions is via the problem of \emph{robust} testing. \gb{More goes here.}

% In order to contextualize our results on the spherical model, we will first address the following question: 
% \begin{center}\emph{What are the reasons to study random geometric graphs?}\end{center}
% \begin{enumerate}
    % \item \emph{Modeling Real-Life Networks:} 
    % Random geometric graphs capture a type of dependence -- edge probabilities that depend on features of the entities represented by nodes -- which occurs in the real world and sciences. Theoretical and empirical results show that geometric graphs fit well certain properties of brain networks \cite{vempala23kcap}, social networks \cite{Almagro22}, and protein-protein interaction networks \cite{higham08}. \textbf{Remark:} We do not claim that any concrete generative model such as \cref{def:sphericalrgg} fits the data perfectly, even if it does so extremely well. 
    % This is an important point that we will return to!
% \end{enumerate}
% The theoretician may still wonder whether there are any benefits to studying random geometric graphs. In particular, \emph{what are the reasons to go beyond the classical $\ergraph$ model of Erd{\H o}s and R\'enyi, in which each edge between $n$ vertices appears {independently} with probability $p?$} 
% \begin{enumerate}
    % \item[2.]\emph{Understanding the Role of Independence in Combinatorial Phenomena:} $\ergraph$ exhibits a variety of deep phenomena, one of the prime examples being generic sharp-thresholds criteria for monotone properties \cite{Friedgut1999SharpTO}. \emph{Are such properties merely a virtue of the independence of edges or they also hold for other distributions?} In \cite{goel05monotoneproperties}, the authors address this question by showing that $n$-vertex random geometric graphs in dimension $d = o(\log n)$ exhibit sharp thresholds for monotone graph properties. 
    % \item[3.]\emph{Combinatorial Constructions:} 
    % While the importance of $\ergraph$ to combinatorial constructions cannot be overstated, starting with the application to Ramsey theory \cite{Erdos1959ER}, the model has limitations. For example, sparse \ERspace are provably not 2-dimensional expanders and a randomized construction for such was only given recently via \emph{random geometric graphs} in dimension $d = \Theta(\log n)$ \cite{Liu22Expander}. 
    % \item[4.]\emph{Statistical Inference With Dependent Data:} Random geometric graphs provide a convenient model for developing tools for learning and estimation from dependent data. Lack of independence makes inference much more challenging but also more realistic due to the non-iid nature of real-life networks. A strikingly simple, but fundamental, question remains open after more than a decade of continuous work and improvements: 
    % \emph{Can one even test for dependence, i.e. test between a random geometric graph and \ERspace}\cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}?    
% \end{enumerate}

% The answers to many of the aforementioned questions on random geometric graphs \emph{depend on the dimension}. Much of the early work (see \cite{penrose03} and references therein) on random geometric graphs focused on low dimensions $d = O(\log n)$ as well as the recent breakthrough on two-dimensional expanders \cite{Liu22Expander}. High-dimension was only considered much more recently, starting with \cite{Devroye11}. The majority of the existing work (\cite{Devroye11} being a notable exception) in this regime so far has focused on the following question: \emph{When is there dependence between the edges of $\RGGsphere?$} When $d\ll (np)^3,$ a simple triangle-based statistic witnesses edge dependence. Conjecturally, when $d\gg (np)^3,$ $\RGGsphere$ converges to $\ergraph$ in total variation distance. Yet, very little is known in the intermediate regime, which raises the question:   
% \begin{center}
%     \textit{Can we characterizes the dependence between edges of $\RGGsphere$ in the regime $\log(n)\ll d\ll (np)^3?$}
% \end{center}
% In the current work, we address this question with an eye towards the aforementioned reasons 1, 2, 3, and 4.
% , which is the focus of the majority of the existing works on \emph{high-dimensional} random geometric graphs thus far, is an important benchmark question. 
% Yet, it does not capture key aspects of the four directions outlined.

% In the current work, we also compare $\RGG$ and \ERspace but   Such a relaxation is motivated by all four reasons to study random geometric graphs that we outlined. 

% Understanding combinatorial phenomena in graphs with dependence between edges explicitly requires the distribution to \emph{not be} \ER. Statistical tasks in non-iid settings (beyond testing for independence) also require a distribution other than \ER. Finally, when modeling complex networks, it is too much to hope that all edges are explained by a simple generative model such as the one in \cref{def:sphericalrgg}. Even ignoring the simplicity of the threshold function $\indicator[\langle\cdot,\cdot\rangle\ge \tau^p_d],$ edges are only determined by pairwise compatibility of the feature vectors and higher-order effects are not captured. Additionally, in real-life networks, (potentially adversarial) corruptions might be present due to malicious entities or non-uniform errors in measurements. Again, testing in total variation is not the correct framework in the presence of corruptions. 

% For example, in social networks, the probability of a friendship may depend on a large variety of factors such as age, geographic location, education, occupation... \footnote{Even though, by no means we claim that any such set of factors fully determines whether there is a friendship. This is an important point that we will return to.} Correlations  

% Random graphs with underlying geometric structure are not only more realistic in modelling real-life networks, but also
% provide a fruitful counterpart to the well-studied \ER model for theoreticians. The dependence among edges leads to genuinely novel combinatorial phenomena (not shared by the simpler \ER model). At the same time, it also makes associated learning and estimation tasks in a non-iid setting much more challenging (but also more realistic due to the non-iid nature of real-life networks).



% Random geometric graphs in low dimension have been extensively studied (see \cite{penrose03} and references therein). The study of the high-dimensional regime in which $d$ grows with $n,$ potentially even at a polynomial rate, however, was more recently initiated by 
% \cite{Devroye11}. In \cite{Devroye11}, the authors discuss both \emph{combinatorial properties} of the distribution, concretely the typical size of the largest clique, as well as \emph{statistical tasks}, namely testing between a random geometric graph and \ER with a single sample. Since then, both directions have flourished. . Determining the regime in which the testing problem is information theoretically possible is still open even though it has witnessed continuous progress  Other statistical tasks have also been studied such as dimension estimation \cite{Bubeck14RGG} and recovering the latent vectors from the graph data \cite{li2023spectral}.  

\subsection{Our Contributions} 
\subsubsection{Our Angle}
We will aim for a characterization of random geometric graphs that allows us to address two previously unexplored themes in the $\log (n)\ll d \ll (np)^3$ regime: \emph{sharp thresholds for edge-monotone properties} and \emph{robustness to bounded edge corruptions.} The combination of \emph{monotonicity} and \emph{edge corruptions} leads us to the following \emph{approximate stochastic dominance} comparison with \ERspace (see also \cite{Liu2022STOC}):
\begin{equation}
\label{eq:couplinquestion}
\tag{Q1}
\begin{split}
    &\textit{When can one couple the two graph distributions in such a way that with high probability}\\
    &\quad\quad\quad\quad\quad\mathsf{G}(n,p(1-\epsilon))\subseteq \RGGsphere \subseteq\mathsf{G}(n,p(1+\epsilon))\textit{ for some small } \epsilon?
    \end{split}
\end{equation}
Here, inclusion is over the edge set. Our main result
is that such a coupling exists if and only if $d\gg np.$ Exploiting this fact, we address aspects of all four of the aforementioned directions:
\begin{enumerate}
    \item \emph{Modeling Real-Life Networks:} Random geometric graphs with few (but otherwise arbitrary) edge corruptions more accurately model real-life networks due to the potential presence of edges not explained by the geometry. These could be due to model misspecifications (it is perhaps too much to hope that all edges are explained by a simple generative model such as the one in \cref{def:sphericalrgg}) or corruptions in the observations due to adversarial interference and measurement errors.
    \item \emph{Understanding the Role of Independence in Combinatorial Phenomena:} We use the \emph{edge-monotonicity} of the coupling to compare monotone properties of $\ergraph$ and $\RGGsphere.$ We give the first proof of sharp thresholds for monotone properties of $\RGG$ in a non-trivial high-dimensional regime.
    \item \emph{Combinatorial Constructions:} A coupling of the form in \cref{eq:couplinquestion} implies a lower bound on the support size of the $\RGGsphere$ distribution. This allows us to use $\RGGsphere$ as a randomized construction for 
    counting the number of geometric graphs in dimension $d.$ 
    \item \emph{Statistical Inference With Dependent Data:} One interpretation of the approximate stochastic dominance is that a sample of $\ergraph$ is a sample of $\RGGsphere$ with $O(\epsilon n^2 p)$ adversarially corrupted edges. This leads us to consider the well-studied question of testing between $\ergraph$ and $\RGGsphere$ \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier} in the previously unexplored setting of adversarial edge-corruptions.  
\end{enumerate}

\subsubsection{Characterizing Edge Dependence in RGG: Main Theorem and Interpretation}
% Motivated by the last consideration -- model mis-specifications and adversarial corruptions -- we choose to study a comparison which allows for a fraction of unexplained edges. Our main theorem is the following algorithmic result.

\begin{theorem}[Main Coupling Result]
\label{thm:algorithmiccoupling}
Consider some $n,d,p$ such that $d= \Omega( \max(np,\log n))$ and $p = \Omega(1/n), p\le 1/2.$ There exists a polynomial-time algorithm which on input $H\sim \ergraph,$ outputs $n$ vectors $V_1 = V_1(H), V_2 = V_2(H), \ldots, V_n = V_n(H)$ in $\dsphere$ with the following two properties:
\begin{enumerate}
    \item The marginal distribution of the vectors is independent uniform: $V_1, V_2, \ldots, V_n\iidsim\unif(\dsphere).$
    \item With high probability (over the input and internal randomness), $\indicator[\langle V_i, V_j\rangle\ge \tau^p_d] = H_{ij}$ for all pairs $i,j$ such that $|\langle V_i, V_j\rangle - \tau_p^d|\ge \frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{3/2}}{d}$ for some absolute constant $c.$
     
\end{enumerate}
\end{theorem}
In other words, the algorithm described above couples $\RGG$ and $\ergraph$ in such a way that they only differ at pairs $(i,j)$ for which $\langle V_i, V_j\rangle $ is very close to the threshold. Elementary calculations shows that with high probability, $G,H$ differ at only $\tilde{O}\Big(\binom{n}{2}p\times\sqrt{\frac{{np}}{d}}\Big) = o\Big(\binom{n}{2}p\Big)$ edges. An immediate implication of \cref{thm:algorithmiccoupling} is the following approximate  stochastic dominance. 

\begin{corollary}[Approximate Stochastic Dominance]
\label{thm:stochasticcoupling}
Consider some $n,d,p$ such that $d= \Omega(np\log^4 n, \log^5n)$ and $p = \Omega(1/n).$ Then, there exists a coupling of $G\sim\RGG(n,\dsphere,p),$ $H_-\sim \mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ and $ H_+\sim \mathsf{G}(n,p(1+\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})),$ 
 such that 
$
H_-\subseteq G \subseteq H_+
$
with high-probability, where inclusion is defined as inclusion over the edge set.
\end{corollary}

In \cite{Liu2022STOC}, the authors prove \cref{thm:stochasticcoupling} under the weaker condition $d \ge \polylog(n)\times n^2p^2$ with the purpose of describing the local structure of random geometric graphs. Our stronger result, based on an entirely different proof technique, is crucial for some of the applications to follow.

Note that $d =\tilde{\Theta}(np)$ is a polynomially smaller dimension than the one required for\linebreak $\TV(\RGGsphere, \ergraph) = o(1),$ For the latter statement to hold, $d= \tilde{\Omega}(n^3p^3)$ is needed as demonstrated by the signed triangle count test \cite{Bubeck14RGG,Liu2022STOC} which is also conjectured to be optimal \cite{Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}. While $d = \tilde{\Theta}(n^3p^3)$ is still rather mysterious, the critical dimension in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} $d = \tilde{\Theta}(np)$ has two natural coalescent interpretations:
\begin{enumerate}
    \item \textbf{Entropic Threshold:} The maximal entropy of a graph with expected density $p$ is $\binom{n}{2}H(p) = \tilde{\Theta}(n^2p)$ and this is achieved by $\ergraph.$ On the other hand, the following heuristic (which we make rigorous in \cref{sec:enumeration}) suggests that the entropy of $\RGGsphere$ is at most $\tilde{\Theta}(nd).$  $\dsphere$ has an $\epsilon$-net of size $\exp(\tilde{O}(d\log(1/\epsilon))).$ 
    Hence, we can discretize the sphere into $\exp(\tilde{O}(d))$ points. As there are $n$ latent vectors $V_1, V_2, \ldots, V_n,$ each effectively of the $\exp(\tilde{O}(d))$-discretization, and the latent vectors uniquely determine the geometric graph, the $\RGGsphere$ distribution effectively has support size 
    $\exp(\tilde{O}(nd)).$ Hence, its entropy is at most $\tilde{O}(nd).$ To match (up to lower order terms) the $\tilde{\Theta}(n^2p)$ entropy of $\ergraph,$ one therefore needs $d = \tilde{\Omega}(np).$ Using \cref{thm:algorithmiccoupling}, in \cref{sec:enumeration} we show that when $d = \tilde{\Omega}(np),$ the support size of $\RGGsphere$ is indeed ``maximal'', i.e. of size $\exp(\tilde{\Omega}(n^2p)).$
    \item \textbf{Spectral Threshold:} Miraculously, as soon as $d \lesssim np,$ there is a spectral separation between $\ergraph$ and $\RGGsphere.$ 
    The second largest eigenvalue of $\ergraph$ is $\tilde{\Theta}(\sqrt{np})$ while the second largest eigenvalue of $\RGGsphere$ is 
    $\tilde{\Theta}({\frac{np}{\sqrt{d}}})\gg \tilde{\Theta}(\sqrt{np})$
    \cite{Liu22Expander,li2023spectral}.
    This spectral separation allows for efficient spectral and SDP algorithms, as in \cite{li2023spectral} and \cref{sec:robusttesting}.
\end{enumerate}

% We will get back to this point in \cref{sec:discussion}, but we believe that the coincidence of entropic and spectral thresholds for the $\RGGsphere$ distributions heuristically explains why no information-computation gaps have been observed for natural statistical tasks such as testing, robust testing, and embedding of random geometric graphs. As soon as there is a very strong information theoretic separation between $\RGG$ and $\ergraph,$ there is also a computationally efficient (spectral) witness.

\begin{remark} We note that in general a relaxed stochastic dominance of the form in \cref{thm:stochasticcoupling} does not guarantee closeness in total variation even if one couples 
$H_-\sim \mathsf{G}(n,p), H_+\sim \mathsf{G}(n,p), G\sim\mathcal{D}$ such that $H_-\subseteq G\subseteq H_+$ with high probability for some $\mathcal{D}.$ Specifically, consider a distribution $\mathcal{D}$ defined by the following coupling. $H_-$ is drawn from $\ergraph.$ Then, $H_+$ is a copy of $H_-$ except that a uniformly random non-edge is changed to an edge. One can check that whenever $p= \Omega(1/n),$ the distribution of $H_+$ is only $o(1)$ TV distance away from $\ergraph.$ Finally, $G$ is the graph among $H_-, H_+$ with an even number of edges. Clearly, $H_-\subseteq G\subseteq H_+$  w.h.p. but $\TV(\mathcal{D}, \ergraph) \ge 1/2 - o(1)$ as the distribution $\mathcal{D}$ is supported on graphs with an even number of edges.
\end{remark}
\subsubsection{Understanding the Role of Independence: Sharp Thresholds} The coupling in \cref{thm:stochasticcoupling} between random geometric graphs and \ERspace is monotone in the sense that 
$
H_-\subseteq G \subseteq H_+.
$
Whenever $H_-\sim \mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ satisfies an increasing property with high probability, so does $G\sim \RGGsphere.$ Whenever 
$G\sim \RGGsphere$ satisfies an increasing property, so does $H_+\sim \mathsf{G}(n,p(1+\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})).$ 
This immediately allows us to translate sharp-threshold phenomena from \ERspace to RGG by considering the couplings between $G_-\subseteq H_-$ 
where 
$G_-\sim \RGG(n,\dsphere,p(1-3\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ and  
$H_+\subseteq G_+ $ where
$G_+\sim \RGG(n,\dsphere,p(1+3\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})).$

\begin{theorem} Suppose that $\mathcal{P}_n$ is a monotone property with critical probability $p^c_n$ which satisfies $p^c_n = \Omega(1/n).$ 
Suppose further that $\mathcal{P}_n$ exhibits a sharp threshold with respect to $\ergraph$ and has a critical window of length $\omega_\epsilon = o(p^c_n).$ 
If $d_n=  \omega(\max(np^c_n\log^4 n, \log^5n)),$ the property $\mathcal{P}_n$ also exhibits a sharp threshold with respect to $\RGG(n,d_n,p)$ and has critical probability $p^c_n + O\Big(p_n^c\frac{\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}\Big)$ and critical window of length 
$\omega_\epsilon  +  O\Big(p_n^c\frac{\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}\Big).$
\end{theorem}

This theorem partially answers in the affirmative a question due to Perkins on whether high-dimensional random geometric graphs exhibit sharp thresholds \cite{perkins2024searching}. 
\subsubsection{Combinatorial Constructions: Enumeration}  \cref{thm:stochasticcoupling} demonstrates that $\RGGsphere$ is a distribution over at least $\exp(\tilde{\Omega}(n^2p))$ graphs when $d= \max(np\log^4 n, \log^5 n).$ The proof is rather simple - if $\mathcal{M}$ is the support of $\RGGsphere,$ using a simple counting argument one can bound the number of graphs that are edge-subgraphs of some graph $H$ in $\mathcal{M}$ and differ from $H$ in $o(\binom{n}{2}p)$ edges. Using this bound, one can arrive at an upper bound for the entropy of $\mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ (which is $\tilde{\Theta}(n^2p)$).  This, in turn, implies a lower bound on $|\mathcal{M}|.$ Altogether, this gives the following result.

\begin{theorem}
\label{thm:enumeration}
The number of graphs which can be realized as intersection graphs of unit spheres in dimension $d$ is at least $\exp(nd\log^{-7}n).$     
\end{theorem}

The statement is tight up to the $\log$ terms as shown in \cite{SAUERMANN2021107593}. The result is not new and sharper estimates (up to the log terms) were recently shown in \cite{SAUERMANN2021107593}. Nevertheless, one advantage of our proof is its simplicity - it is based on a natural probabilistic construction, spherical random geometric graphs. The techniques from algebraic geometry and algebraic topology in \cite{SAUERMANN2021107593} are significantly more involved, even though admittedly much more systematic and sharper.

\subsubsection{Inference with Dependent Data: Robust Testing} One immediate application of \cref{thm:stochasticcoupling} is  the following. Suppose that 
$\epsilon\in (0,1]$ is a small fixed constant. Whenever $d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5)$ (where $K(\epsilon)$ depends solely on $\epsilon$), one can with high probability (adversarially) corrupt $\epsilon \binom{n}{2}p$ edges of a sample from $\RGGsphere$ and produce a sample from $\ergraph.$
Hence, the following robust testing problem is information-theoretically impossible when $d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5):$ 
\begin{problem}[Robust Testing of Geometry With Edge Corruptions]
\label{problem:robusttesting}
Given are $n,d\in \mathbb{N},$ $p\in [0,1]$ and a fixed constant $\epsilon.$
Consider the following hypothesis testing problem. One observes a graph $H$ and needs to decide between $H_0: H = \mathcal{A}(\bfG),\bfG\sim \ergraph$ and 
$H_1: H = \mathcal{A}(\bfG),\bfG\sim \mathsf{RGG}(n,d,p).$ Here $\mathcal{A}$ is an arbitrary adversary who is allowed to corrupt at most $\epsilon \binom{n}{2}p$ edges and non-edges.
\end{problem}
We restrict the adversary to changing $\epsilon \binom{n}{2}p$ edges for a small constant $\epsilon$ as the robust testing problem is otherwise trivially impossible. Both $\mathsf{RGG}(n,d,p)$ and 
$\ergraph$ have with high probability $1.5\binom{n}{2}p$ edges. Hence, an adversary $
\mathcal{A}$ who simply deletes all edges of a sample from $\RGG$ and then inserts Bernoulli $p$ edges (in total $3\binom{n}{2}p$ w.h.p.) can transform into a sample from $\ergraph.$ Thus, \cref{problem:robusttesting} captures the setting of ``maximal adversaries.'' 

\begin{remark}[Efficient adversaries]
\label{rmk:eficientadversary}
When $d = o((np)^3(\log n)^3), d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5)),$ \cref{problem:robusttesting} is information theoretically impossible even against polynomial-time adversaries. In this regime, an adversary can see a sample $H$ and (correctly with high probability) test using the signed-triangle statistic \cite{Liu2022STOC} whether the sample is from $\ergraph$ or $\RGGsphere.$ If $H$ is from $\ergraph,$ the adversary can use the efficient algorithm from \cref{thm:algorithmiccoupling} and produce (with high-probability) a sample from $\RGGsphere$ differing from $H$ only at $o\Big(\binom{n}{2}p\Big)$ edges. If $H$ is from $\RGG$ already, the adversary does not change edges. 
\end{remark}



Due to the miraculous coincidence of spectral and entropic thresholds, \cref{problem:robusttesting} is solvable in polynomial time even against computationally unbounded adversaries when $d\ll np.$ 

\begin{theorem}
\label{thm:robustestingsos}
There exists some constant absolute constant $K_r>0$ with the following property. When $d\le K_r\min(np\log(1/p), n^2p^2\log(1/p)\log^{-2}n)$ and $d = \omega(\log 1/p),$ there exists a polynomial-time algorithm solving \cref{problem:robusttesting} with high probability for all $\epsilon\le K_r.$
\end{theorem}
We overview the algorithm in \cref{sec:nontechnicalrobust} and give full detail in \cref{sec:robusttesting}. It is a constant degree SoS program for spectral refutation of a small operator norm of the centered adjacency matrix. The key insight, implicit in \cite{li2023spectral}, is that the latent vectors witness a large second eigenvalue for a random geometric graph. The approach works for robust testing against any null hypothesis with a substantially smaller second eigenvalue than $\RGGsphere,$ see \cref{rmk:testingrobustly}.

\begin{remark}
\label{rmk:couplingimpossibilityfromspectral}
\cref{thm:robustestingsos} implies that when $d \le K_r\min(np\log(1/p), n^2p^2\log(1/p)\log^{-2}n),$ there does not exist a coupling between $H_-\sim \mathsf{G}(n,p(1-o(1)),G\sim \RGGsphere, H_+\sim \mathsf{G}(n,p(1+o(1))$
such that $H_-\subseteq G\subseteq H_+$ w.h.p. Otherwise, one can use this coupling as an adversary for \cref{problem:robusttesting} even against computationally-unbounded testers but \cref{thm:robustestingsos} shows that such an adversary cannot exist. Hence, the dimension requirement $d = \tilde{\Omega}(np)$ in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} is tight (up to $\polylog$ factors).
\end{remark}



\subsection{Prior Work and Challenges}
\paragraph{Coupling Random Geometric Graphs and \ER.} In \cite{Liu2022STOC}, the authors prove \cref{thm:stochasticcoupling} under the weaker condition $d\ge n^2p^2\log^4n.$ In their construction, they sample $V_1, V_2, \ldots, V_n$ sequentially. A caricature of their argument is that with high probability, when sampling $V_1, V_2, \ldots, V_{k-1}$ the intersection of any $i\approx pk$ $p$-caps and $k-i-1\approx k(1-p)$ $p$-anti-caps corresponding to $V_1, V_2, \ldots, V_{i-1}$\footnote{For $V\in \dsphere,$ the associated $p$-cap is the set $\{U \in \dsphere\; : \langle U, V\rangle\ge \tau^p_d\}$  and the $p$-anti-cap is its complement} is sufficiently close to $p^{i}(1-p)^{k-i-1}.$ Hence, one should expect that the edges from $k$ to $[k-1]$ roughly are distributed as ``independent'' $\Bernoulli(p)$ variables. They make this statement precise by quantifying ``sufficiently close'' via a concentration argument based on transportation inequalities. While our proof of \cref{thm:stochasticcoupling} is entirely different, it suggests what might be suboptimal in the approach of \cite{Liu2022STOC}. Typical intersections of $\approx pk$ caps and $k-i-1\approx k(1-p)$ anti-caps might concentrate much better than worst-case 
intersections due to a square-root cancellation phenomenon. We use this idea in our proof to get $d\ge \max(np, \log n)$ and if we consider \emph{all} intersections of caps and anti-caps instead, we also obtain a result for $d\ge n^2p^2\polylog n.$ While the square-root cancellation comes naturally in our martingale-based analysis, it is unclear whether it can be incorporated in the transportation-based approach of \cite{Liu2022STOC}. Even beyond that, an advantage of our approach is that there is an efficient algorithm producing the coupling -- \cref{thm:algorithmiccoupling}. The result of \cite{Liu2022STOC} is not obviously algorithmically efficient as it requires keeping track of an intersection of caps and anti-caps on the sphere and being able to sample and estimate the volume of this intersection.    

A different work which shows that in certain regimes random geometric graphs can be represented as $\ergraph$ with some planted structure (i.e. the edges on locations for which $|\langle V_i, V_j\rangle - \tau_p^d|\le \frac{\sqrt{np\log n}}{d}$ in \cref{thm:algorithmiccoupling}) is 
\cite{bangachev2024fourier}. In fact, in their representation, again the non-\ERspace pairs $(i,j)$ are exactly the ones for which $\langle V_i, V_j\rangle$ are close to $\tau^p_d$ (called \emph{fragile pairs} in \cite{bangachev2024fourier}). While some of our ideas are related to and motivated by \cite{bangachev2024fourier}, there is a fundamental barrier to their proof technique. It crucially relies on performing the Gram-Schmidt operation on the latent vectors\footnote{To be fully precise, the Gram-Schmidt is performed on the isotropic Gaussian vectors $Z_1, Z_2, \ldots, Z_n.$ 
% where $Z_i = V_i \chi_i$ (where $\chi_i$ is an appropriate square root of a $\chi^2$ random variable). 
This, however, makes little difference to the arguments in \cite{bangachev2024fourier} and the current work, see \cref{rmk:sphericaltogaussian}.} $V_1, V_2, \ldots, V_n.$ In particular, this method requires $d\ge n,$ so obtaining a result of the form in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} for $d\ll n$ is impossible. 

\paragraph{Testing.} To the best of our knowledge, this work is the first to study the robust testing problem between $\RGGsphere$ and \ER. The same question in the setting of no edge corruptions has attracted significant attention in recent years \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}. Formally, one observes a graph $G$ and needs to decide $H_0:G\sim \ergraph$ or $H_1:G\sim \RGGsphere.$ By counting signed triangles, i.e computing $\sum_{i<j<k}(G_{ij} - p)(G_{jk}-p)(G_{ki}-p),$ one can succeed with high probability whenever $d = \omega(n^3p^3\log^3(1/p))$ \cite{Bubeck14RGG,Schramm_2022}.  The current state-of-the-art information-theoretic lower bounds are that when $d\ge (\log n)^C n^3p^2,$ the problem is information theoretically impossible as well as when 
$p = \Theta(1/n)$ and $d\ge (\log n)^C$ for some constant $C$ \cite{Liu2022STOC}. Even ignoring $\polylog $ factors, there is still a $1/p$ gap between the testing algorithm and the information-theoretic lower bound when $1/n\ll p\ll 1/2.$ The gap was recently closed with respect to low-degree polynomial tests by \cite{bangachev2024fourier}: counting signed triangles is optimal among all degree $\log^{2-\epsilon} n$ polynomial tests.

We note that both the question of upper and lower-bounds are significantly different when one considers the testing problem with a constant number of adversarial corruptions as in \cref{problem:robusttesting}. On the algorithmic side, simple counting tests such as counting signed triangles necessarily fail. For example, the expected number of signed triangles in $\RGGsphere$ is $\tilde{\Theta}(n^3p^3/\sqrt{d})$ \cite{Liu2022STOC}. One can increase the expected number of signed triangles in $\ergraph$ by planting a clique of size $\tilde{O}(np/d^{1/6})$ which requires $\tilde{O}(n^2p^2/d^{1/3}) = o(n^2p)$ adversarial corruptions. One can argue similarly for other subgraph-counting tests. This is why we need a more sophisticated sum-of-squares spectral refutation algorithm which uses the true embedding as a witness. To the best of our knowledge, \cite{mao2024informationtheoretic} is the only other work which uses an embedding-based approach for testing for random geometric graphs, but their work is in low-dimension and the algorithm is not computationally efficient. Regarding lower-bounds, all of the prior work on the setting without adversarial corruptions \cite{Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC} very strongly exploits distributional assumptions (such as the relationship to Wishart ensembles and a certain $\KL$-convexity argument revealing the latent vectors). We do not expect that any of these techniques applies to the adversarial setting. Instead, we rely on our coupling argument \cref{thm:stochasticcoupling}.

Finally, there is still a gap between the known upper-bound $\tilde{\Theta}(n^3p^3)$ and the lower-bound $\Tilde{\Theta}(n^3p^2)$ in the setting of no corruptions when $p = \omega(1/n).$ In this work, we determine that (up to log factors) $d = \Tilde{\Theta}(np)$ is the tight threshold for testing with adversarial corruptions computationally and information-theoretically. Part of the reason for this difference between the robust setting and the setting without corruptions is how well we understand the respective thresholds. $d = \Tilde{\Theta}(np)$ has a very clear significance - as an entropic threshold information-theoretically and as a spectral threshold computationally. Yet, the condition $d = \Tilde{\Theta}(n^3p^3)$ so far seems to only have a computational interpretation. It is the threshold below which one can test counting signed triangles, which are ``the most informative subgraph'' among $\log^{2-\epsilon}n$-sized subgraphs \cite{bangachev2024fourier}. The search for the correct information-theoretic interpretation of  $d = \Tilde{\Theta}(n^3p^3)$ remains open.

\paragraph{Sharp Thresholds.} The question of whether monotone properties exhibit sharp thresholds is by far the best understood in the case of product distributions. The seminal paper of \cite{Friedgut1999SharpTO} establishes very broad conditions on vertex-transitive properties for which the \ERspace distribution exhibits sharp-thresholds. In non-product settings, much less is understood. Important progress has been made in the case of measures satisfying the FKG lattice property \cite{grimmett2006random}. However,
this property does not seem to hold obviously for random geometric graphs.
In the case of low-dimensional random geometric graphs (over the solid cube $[0,1]^d$), \cite{goel05monotoneproperties} show sharp-thresholds phenomena by proving that if $G_1, G_2$ are independent samples with densities $p(1-o(1)),p,$ then $G_1\subseteq G_2$ with high probability. The work of \cite{Bradonjic2013OnST} also deals with sharp thresholds on random geometric graphs, but again only applies to low dimensions. The methods of \cite{goel05monotoneproperties,Bradonjic2013OnST} do not seem applicable to the high-dimensional setting because both rely on the fact that a very fine (grid) subdivision of the space is well-covered by the latent vectors. In $d$ dimensions, the subdivision has $\exp(\Omega(d))$ cells, which is much larger than $n$ when $d = \omega(\log n).$
 
To the best of our knowledge, our result is the first to prove a generic sharp-thresholds statement for high-dimensional random geometric graphs in a non-trivial regime (i.e., when $\RGGsphere$ is not asymptotically the product distribution $\ergraph$ in total variation distance). 

\paragraph{Enumeration.} A classic result in algebraic geometry due to Warren \cite{warren1968lowerbounds} nearly immediately implies that the number of geometric graphs in $d$ dimensions is at most $(Cn/d)^{dn}$ for some explicit constant $C$ when $d = o(n)$ \cite{MCDIARMID2011627,SAUERMANN2021107593}. The main idea is that the edges of a geometric graph correspond to the sign patterns of $\binom{n}{2}$ polynomials over the $dn$ variables $\{(v_i)_j\}_{1\le i \le n, 1\le j \le d}.$ The variables are the coordinates of the latent vectors and the polynomials are the squared pairwise $\ell_2$ distance minus the radius squared.

Proving lower bounds, however, turns out to be a much more challenging task. In \cite{MCDIARMID2011627}, it is shown that in 2 dimensions the number of geometric graphs (known also as unit disk graphs in this case) is $n^{(2+o(1))n}.$ Using more sophisticated tools from algebraic geometry and topology, \cite{SAUERMANN2021107593} shows that the number of 
geometric graphs  in $d$ dimensions is $n^{(d+o(1))n}$ when $d = o(n).$

While our proof loses a non-trivial poly-logarithmic factor in the exponent, it is much simpler and relies on a simple probabilistic construction - spherical random geometric graphs.

\paragraph{Other Works on Random Geometric Graphs in The Regime $\log(n)\ll d\ll (np)^3.$} In \cite{Devroye11}, the authors show that as long as $d\gg \polylog(n), $ the clique numbers of $\ergraph$ and $\RGGsphere$ are essentially the same. While their work is also focused on a comparison with \ERspace in a metric other than total variation distance, one major difference is that it is only for a single (monotone) property, the clique number. Our coupling result addresses \emph{all} monotone properties.   

\subsection{Organization}
In \cref{sec:preliminaries} we introduce some basic preliminaries and notation. In \cref{sec:nontechnical}, we give non-technical overviews of our two main algorithmic results: the coupling algorithm in \cref{thm:algorithmiccoupling} and the spectral refutation algorithm in \cref{thm:robustestingsos}. We give the full details in respectively \cref{sec:coupling} and \cref{sec:robusttesting}. In \cref{sec:enumeration} we prove \cref{thm:enumeration} via a rather simple counting argument using \cref{thm:algorithmiccoupling}. We end with several remarks and open questions regarding our results in \cref{sec:discussion}.




==> IntroductionV4.tex <==
% \section{Introduction}
% \begin{enumerate}
%     \item RGG is important: ``realistic" model (triangles etc.). RGG is mathematically interesting. Latent space graphs, Aldous-Hoover, old references on latent space graphs 1970, graphons. (The edge probabilities in social, biological, communication networks depend on features of the entities represented by nodes. Theoretical and empirical results show that geometric graphs fit well certain properties of brain networks \cite{vempala23kcap}, social networks \cite{Almagro22}, and protein-protein interaction networks \cite{higham08}.)
%     \item Define RGG -- MOST CANONICAL MODEL
%     \item The whole point of the model is that the edges are dependent. It turns out that for $d\gg (np)^3$, the model is conjectured to be close in TV to ER, therefore this is in some sense the completely uninteresting regime. When $\mathrm{\polylog}(n)\ll d \ll (np)^3$, very little is understood about the model. 
%     \item In low dimensions several striking phenomena.  HDX. 
%     \item Other properties such as spectral radius and clique number have various thresholds in $d$ that are far below the threshold for TV convergence. 
%     \item We ask to what extent do various characteristics and/or properties for ER hold for RGG? And for properties that RGG does have, can we determine the precise threshold in dimension? Where to start? In this paper we aim for general phenomena and graph properties.
%     \item One of the most fundamental features of ER graph is sharp threshold phenomenon for monotone graph properties. For RGG in quite low dimension, sharp thresholds. Completely mysterious in higher dimension. Even the connectivity threshold of RGG is not at all obvious. Similarly, not only the clique number, but counts of subgraphs (give some references as to why this is a big deal in combinatorics, rich literature).  
%     \item The question of whether RGG and ER are the same is TV. The question of whether RGG and ER are \emph{not too different} is Wasserstein. Just as TV is equivalent to \emph{hypothesis testing}, Wasserstein corresponds to a certain formulation of \emph{robust testing}. Model misspecification is an inevitability in statistical modeling and is needed to address the efficacy of real-world algorithms. 
    
%     % \item At high level, much of the work on high-dimensional random geometric graphs can be interpreted as comparing RGG to ER in some way. The interesting thing here is that there is a threshold dimension at which the model resembles or differs from ER. 
% \end{enumerate}

% \newpage
\section{Introduction}
% Random graphs have been a fundamental object of study since the seminal paper of Erd{\H o}s and R\'enyi \cite{Erdos1959ER}. In the \ERspace model $\ergraph,$ each edge among $n$ vertices appears independently with probability $p.$ More than 80 years of systematic study have revealed many marvels of the $\ergraph$ model. These have been instrumental to major developments in combinatorics, algorithm design and complexity, and network modeling. \emph{But what if we want to model dependence between edges? And why would we do so?} 

% \paragraph{1. Modeling Dependence via Random Geometric Graphs.}
Random geometric graphs have emerged as a fruitful way to model dependence between edges in random networks in both theory and practice \cite{penrose03}. Random geometric graphs capture the simple but omnipresent phenomenon that larger similarity in certain characteristics increases the likelihood of connection.   Random geometric graphs capture a type of dependence -- edge probabilities that depend on features of the entities represented by nodes -- which occurs in the real world and sciences. Theoretical and empirical results show that geometric graphs fit well certain properties of brain networks \cite{vempala23kcap}, social networks \cite{Almagro22}, and protein-protein interaction networks \cite{higham08}. 
% \textbf{Remark:} We do not claim that any concrete generative model such as \cref{def:sphericalrgg} fits the data perfectly, even if it does so extremely well. 
\cite{mcfarland1973social,mcpherson2001birds,hoff2002latent}. 

Perhaps the most canonical instance is the \emph{Spherical Random Geometric Graph}. 

\begin{definition}[Spherical Random Geometric Graph]
\label{def:sphericalrgg}
A sample from the distribution $\RGGsphere$ over graphs on $n$ vertices $[n] = \{1,\ldots, n\}$ of
dimension $d$ with expected density $p$ is generated as follows. First, $n$ vectors $V_1,  \ldots, V_n$ are drawn independently from the uniform distribution on the sphere $\dsphere.$ Then, an edge between $i$ and $j$ is formed if and only if $\langle V_i ,V_j\rangle \ge \tau^p_d.$ Here, $\tau^p_d$ is chosen so that $p = \prob[\langle V_i ,V_j\rangle \ge \tau^p_d].$ 
\end{definition}


% The theoretician may still wonder whether there are any benefits to studying random geometric graphs. 

% In particular, \emph{what are the reasons to go beyond the classical $\ergraph$ model of Erd{\H o}s and R\'enyi, in which each edge between $n$ vertices appears {independently} with probability $p?$} 
To give context for our results, we mention several fascinating directions in the study of RGG. All of these can be interpreted as a sort of comparison between RGG and \ER. 
\begin{enumerate}
    \item \emph{Understanding the Role of Independence in Combinatorial Phenomena:} $\ergraph$ exhibits a variety of deep phenomena, one of the prime examples being generic criteria for sharp-thresholds of monotone properties \cite{Friedgut1999SharpTO}. \emph{Which \ERspace phenomena hold also for RGG?} In \cite{goel05monotoneproperties}, the authors address this question by showing that $n$-vertex random geometric graphs in dimension $d = o(\log n)$ exhibit sharp thresholds for monotone graph properties. The question remains open in higher dimension. 
    \item \emph{Combinatorial Constructions:} 
    While the importance of $\ergraph$ to combinatorial constructions cannot be overstated, starting with the application to Ramsey theory \cite{Erdos1959ER}, the model has limitations. For example, sparse \ERspace are provably not 2-dimensional expanders and a randomized construction for such was only given recently via \emph{random geometric graphs} in dimension $d = \Theta(\log n)$ \cite{Liu22Expander}. 
    \item \emph{Statistical Inference With Dependent Data:} Random geometric graphs provide a convenient model for developing tools for learning and estimation from dependent data. Lack of independence makes inference much more challenging but also more realistic due to the non-iid nature of real-life networks. A strikingly simple, but fundamental, question remains open after more than a decade of continuous work and improvements: 
    \emph{Can one even test for dependence, i.e. test between a random geometric graph and \ERspace}\cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}?    
\end{enumerate}

The answers to many of the aforementioned questions on random geometric graphs \emph{depend on the dimension}. Much of the early work (see \cite{penrose03} and references therein) on random geometric graphs focused on low dimensions $d = O(\log n)$ as well as the recent breakthrough on two-dimensional expanders \cite{Liu22Expander}. High-dimension was only considered much more recently, starting with \cite{Devroye11}. The majority of the existing work (\cite{Devroye11} being a notable exception) in this regime so far has focused on the following question: \emph{When is there dependence between the edges of $\RGGsphere?$} When $d\ll (np)^3,$ a simple triangle-based statistic witnesses edge dependence. Conjecturally, when $d\gg (np)^3,$ $\RGGsphere$ converges to $\ergraph$ in total variation distance. Yet, very little is known in the intermediate regime, which raises the question:   
\begin{center}
    \textit{Can we characterizes the dependence between edges of $\RGGsphere$ in the regime $\log(n)\ll d\ll (np)^3?$}
\end{center}
In the current work, we address this question with an eye towards the aforementioned reasons 1, 2, 3, and 4.
% , which is the focus of the majority of the existing works on \emph{high-dimensional} random geometric graphs thus far, is an important benchmark question. 
% Yet, it does not capture key aspects of the four directions outlined.

% In the current work, we also compare $\RGG$ and \ERspace but   Such a relaxation is motivated by all four reasons to study random geometric graphs that we outlined. 

% Understanding combinatorial phenomena in graphs with dependence between edges explicitly requires the distribution to \emph{not be} \ER. Statistical tasks in non-iid settings (beyond testing for independence) also require a distribution other than \ER. Finally, when modeling complex networks, it is too much to hope that all edges are explained by a simple generative model such as the one in \cref{def:sphericalrgg}. Even ignoring the simplicity of the threshold function $\indicator[\langle\cdot,\cdot\rangle\ge \tau^p_d],$ edges are only determined by pairwise compatibility of the feature vectors and higher-order effects are not captured. Additionally, in real-life networks, (potentially adversarial) corruptions might be present due to malicious entities or non-uniform errors in measurements. Again, testing in total variation is not the correct framework in the presence of corruptions. 

% For example, in social networks, the probability of a friendship may depend on a large variety of factors such as age, geographic location, education, occupation... \footnote{Even though, by no means we claim that any such set of factors fully determines whether there is a friendship. This is an important point that we will return to.} Correlations  

% Random graphs with underlying geometric structure are not only more realistic in modelling real-life networks, but also
% provide a fruitful counterpart to the well-studied \ER model for theoreticians. The dependence among edges leads to genuinely novel combinatorial phenomena (not shared by the simpler \ER model). At the same time, it also makes associated learning and estimation tasks in a non-iid setting much more challenging (but also more realistic due to the non-iid nature of real-life networks).



% Random geometric graphs in low dimension have been extensively studied (see \cite{penrose03} and references therein). The study of the high-dimensional regime in which $d$ grows with $n,$ potentially even at a polynomial rate, however, was more recently initiated by 
% \cite{Devroye11}. In \cite{Devroye11}, the authors discuss both \emph{combinatorial properties} of the distribution, concretely the typical size of the largest clique, as well as \emph{statistical tasks}, namely testing between a random geometric graph and \ER with a single sample. Since then, both directions have flourished. . Determining the regime in which the testing problem is information theoretically possible is still open even though it has witnessed continuous progress  Other statistical tasks have also been studied such as dimension estimation \cite{Bubeck14RGG} and recovering the latent vectors from the graph data \cite{li2023spectral}.  

\subsection{Our Contributions} 
\subsubsection{Our Angle}
We will aim for a characterization of random geometric graphs that allows us to address two previously unexplored themes in the $\log (n)\ll d \ll (np)^3$ regime: \emph{sharp thresholds for edge-monotone properties} and \emph{robustness to bounded edge corruptions.} The combination of \emph{monotonicity} and \emph{edge corruptions} leads us to the following \emph{approximate stochastic dominance} comparison with \ERspace (see also \cite{Liu2022STOC}):
\begin{equation}
\label{eq:couplinquestion}
\tag{Q1}
\begin{split}
    &\textit{When can one couple the two graph distributions in such a way that with high probability}\\
    &\quad\quad\quad\quad\quad\mathsf{G}(n,p(1-\epsilon))\subseteq \RGGsphere \subseteq\mathsf{G}(n,p(1+\epsilon))\textit{ for some small } \epsilon?
    \end{split}
\end{equation}
Here, inclusion is over the edge set. Our main result
is that such a coupling exists if and only if $d\gg np.$ Exploiting this fact, we address aspects of all four of the aforementioned directions:
\begin{enumerate}
    \item \emph{Modeling Real-Life Networks:} Random geometric graphs with few (but otherwise arbitrary) edge corruptions more accurately model real-life networks due to the potential presence of edges not explained by the geometry. These could be due to model misspecifications (it is perhaps too much to hope that all edges are explained by a simple generative model such as the one in \cref{def:sphericalrgg}) or corruptions in the observations due to adversarial interference and measurement errors.
    \item \emph{Understanding the Role of Independence in Combinatorial Phenomena:} We use the \emph{edge-monotonicity} of the coupling to compare monotone properties of $\ergraph$ and $\RGGsphere.$ We give the first proof of sharp thresholds for monotone properties of $\RGG$ in a non-trivial high-dimensional regime.
    \item \emph{Combinatorial Constructions:} A coupling of the form in \cref{eq:couplinquestion} implies a lower bound on the support size of the $\RGGsphere$ distribution. This allows us to use $\RGGsphere$ as a randomized construction for 
    counting the number of geometric graphs in dimension $d.$ 
    \item \emph{Statistical Inference With Dependent Data:} One interpretation of the approximate stochastic dominance is that a sample of $\ergraph$ is a sample of $\RGGsphere$ with $O(\epsilon n^2 p)$ adversarially corrupted edges. This leads us to consider the well-studied question of testing between $\ergraph$ and $\RGGsphere$ \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier} in the previously unexplored setting of adversarial edge-corruptions.  
\end{enumerate}

\subsubsection{Characterizing Edge Dependence in RGG: Main Theorem and Interpretation}
% Motivated by the last consideration -- model mis-specifications and adversarial corruptions -- we choose to study a comparison which allows for a fraction of unexplained edges. Our main theorem is the following algorithmic result.

\begin{theorem}[Main Coupling Result]
\label{thm:algorithmiccoupling}
Consider some $n,d,p$ such that $d= \Omega( \max(np,\log n))$ and $p = \Omega(1/n), p\le 1/2.$ There exists a polynomial-time algorithm which on input $H\sim \ergraph,$ outputs $n$ vectors $V_1 = V_1(H), V_2 = V_2(H), \ldots, V_n = V_n(H)$ in $\dsphere$ with the following two properties:
\begin{enumerate}
    \item The marginal distribution of the vectors is independent uniform: $V_1, V_2, \ldots, V_n\iidsim\unif(\dsphere).$
    \item With high probability (over the input and internal randomness), $\indicator[\langle V_i, V_j\rangle\ge \tau^p_d] = H_{ij}$ for all pairs $i,j$ such that $|\langle V_i, V_j\rangle - \tau_p^d|\ge \frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{3/2}}{d}$ for some absolute constant $c.$
     
\end{enumerate}
\end{theorem}
In other words, the algorithm described above couples $\RGG$ and $\ergraph$ in such a way that they only differ at pairs $(i,j)$ for which $\langle V_i, V_j\rangle $ is very close to the threshold. Elementary calculations shows that with high probability, $G,H$ differ at only $\tilde{O}\Big(\binom{n}{2}p\times\sqrt{\frac{{np}}{d}}\Big) = o\Big(\binom{n}{2}p\Big)$ edges. An immediate implication of \cref{thm:algorithmiccoupling} is the following approximate  stochastic dominance. 

\begin{corollary}[Approximate Stochastic Dominance]
\label{thm:stochasticcoupling}
Consider some $n,d,p$ such that $d= \Omega(np\log^4 n, \log^5n)$ and $p = \Omega(1/n).$ Then, there exists a coupling of $G\sim\RGG(n,\dsphere,p),$ $H_-\sim \mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ and $ H_+\sim \mathsf{G}(n,p(1+\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})),$ 
 such that 
$
H_-\subseteq G \subseteq H_+
$
with high-probability, where inclusion is defined as inclusion over the edge set.
\end{corollary}

In \cite{Liu2022STOC}, the authors prove \cref{thm:stochasticcoupling} under the weaker condition $d \ge \polylog(n)\times n^2p^2$ with the purpose of describing the local structure of random geometric graphs. Our stronger result, based on an entirely different proof technique, is crucial for some of the applications to follow.

Note that $d =\tilde{\Theta}(np)$ is a polynomially smaller dimension than the one required for\linebreak $\TV(\RGGsphere, \ergraph) = o(1),$ For the latter statement to hold, $d= \tilde{\Omega}(n^3p^3)$ is needed as demonstrated by the signed triangle count test \cite{Bubeck14RGG,Liu2022STOC} which is also conjectured to be optimal \cite{Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}. While $d = \tilde{\Theta}(n^3p^3)$ is still rather mysterious, the critical dimension in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} $d = \tilde{\Theta}(np)$ has two natural coalescent interpretations:
\begin{enumerate}
    \item \textbf{Entropic Threshold:} The maximal entropy of a graph with expected density $p$ is $\binom{n}{2}H(p) = \tilde{\Theta}(n^2p)$ and this is achieved by $\ergraph.$ On the other hand, the following heuristic (which we make rigorous in \cref{sec:enumeration}) suggests that the entropy of $\RGGsphere$ is at most $\tilde{\Theta}(nd).$  $\dsphere$ has an $\epsilon$-net of size $\exp(\tilde{O}(d\log(1/\epsilon))).$ 
    Hence, we can discretize the sphere into $\exp(\tilde{O}(d))$ points. As there are $n$ latent vectors $V_1, V_2, \ldots, V_n,$ each effectively of the $\exp(\tilde{O}(d))$-discretization, and the latent vectors uniquely determine the geometric graph, the $\RGGsphere$ distribution effectively has support size 
    $\exp(\tilde{O}(nd)).$ Hence, its entropy is at most $\tilde{O}(nd).$ To match (up to lower order terms) the $\tilde{\Theta}(n^2p)$ entropy of $\ergraph,$ one therefore needs $d = \tilde{\Omega}(np).$ Using \cref{thm:algorithmiccoupling}, in \cref{sec:enumeration} we show that when $d = \tilde{\Omega}(np),$ the support size of $\RGGsphere$ is indeed ``maximal'', i.e. of size $\exp(\tilde{\Omega}(n^2p)).$
    \item \textbf{Spectral Threshold:} Miraculously, as soon as $d \lesssim np,$ there is a spectral separation between $\ergraph$ and $\RGGsphere.$ 
    The second largest eigenvalue of $\ergraph$ is $\tilde{\Theta}(\sqrt{np})$ while the second largest eigenvalue of $\RGGsphere$ is 
    $\tilde{\Theta}({\frac{np}{\sqrt{d}}})\gg \tilde{\Theta}(\sqrt{np})$
    \cite{Liu22Expander,li2023spectral}.
    This spectral separation allows for efficient spectral and SDP algorithms, as in \cite{li2023spectral} and \cref{sec:robusttesting}.
\end{enumerate}

% We will get back to this point in \cref{sec:discussion}, but we believe that the coincidence of entropic and spectral thresholds for the $\RGGsphere$ distributions heuristically explains why no information-computation gaps have been observed for natural statistical tasks such as testing, robust testing, and embedding of random geometric graphs. As soon as there is a very strong information theoretic separation between $\RGG$ and $\ergraph,$ there is also a computationally efficient (spectral) witness.

\begin{remark} We note that in general a relaxed stochastic dominance of the form in \cref{thm:stochasticcoupling} does not guarantee closeness in total variation even if one couples 
$H_-\sim \mathsf{G}(n,p), H_+\sim \mathsf{G}(n,p), G\sim\mathcal{D}$ such that $H_-\subseteq G\subseteq H_+$ with high probability for some $\mathcal{D}.$ Specifically, consider a distribution $\mathcal{D}$ defined by the following coupling. $H_-$ is drawn from $\ergraph.$ Then, $H_+$ is a copy of $H_-$ except that a uniformly random non-edge is changed to an edge. One can check that whenever $p= \Omega(1/n),$ the distribution of $H_+$ is only $o(1)$ TV distance away from $\ergraph.$ Finally, $G$ is the graph among $H_-, H_+$ with an even number of edges. Clearly, $H_-\subseteq G\subseteq H_+$  w.h.p. but $\TV(\mathcal{D}, \ergraph) \ge 1/2 - o(1)$ as the distribution $\mathcal{D}$ is supported on graphs with an even number of edges.
\end{remark}
\subsubsection{Understanding the Role of Independence: Sharp Thresholds} The coupling in \cref{thm:stochasticcoupling} between random geometric graphs and \ERspace is monotone in the sense that 
$
H_-\subseteq G \subseteq H_+.
$
Whenever $H_-\sim \mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ satisfies an increasing property with high probability, so does $G\sim \RGGsphere.$ Whenever 
$G\sim \RGGsphere$ satisfies an increasing property, so does $H_+\sim \mathsf{G}(n,p(1+\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})).$ 
This immediately allows us to translate sharp-threshold phenomena from \ERspace to RGG by considering the couplings between $G_-\subseteq H_-$ 
where 
$G_-\sim \RGG(n,\dsphere,p(1-3\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ and  
$H_+\subseteq G_+ $ where
$G_+\sim \RGG(n,\dsphere,p(1+3\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}})).$

\begin{theorem} Suppose that $\mathcal{P}_n$ is a monotone property with critical probability $p^c_n$ which satisfies $p^c_n = \Omega(1/n).$ 
Suppose further that $\mathcal{P}_n$ exhibits a sharp threshold with respect to $\ergraph$ and has a critical window of length $\omega_\epsilon = o(p^c_n).$ 
If $d_n=  \omega(\max(np^c_n\log^4 n, \log^5n)),$ the property $\mathcal{P}_n$ also exhibits a sharp threshold with respect to $\RGG(n,d_n,p)$ and has critical probability $p^c_n + O\Big(p_n^c\frac{\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}\Big)$ and critical window of length 
$\omega_\epsilon  +  O\Big(p_n^c\frac{\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}\Big).$
\end{theorem}

This theorem partially answers in the affirmative a question due to Perkins on whether high-dimensional random geometric graphs exhibit sharp thresholds \cite{perkins2024searching}. 
\subsubsection{Combinatorial Constructions: Enumeration}  \cref{thm:stochasticcoupling} demonstrates that $\RGGsphere$ is a distribution over at least $\exp(\tilde{\Omega}(n^2p))$ graphs when $d= \max(np\log^4 n, \log^5 n).$ The proof is rather simple - if $\mathcal{M}$ is the support of $\RGGsphere,$ using a simple counting argument one can bound the number of graphs that are edge-subgraphs of some graph $H$ in $\mathcal{M}$ and differ from $H$ in $o(\binom{n}{2}p)$ edges. Using this bound, one can arrive at an upper bound for the entropy of $\mathsf{G}(n,p(1-\frac{c\max(\sqrt{np}, \sqrt{\log n})(\log n)^{2}}{\sqrt{d}}))$ (which is $\tilde{\Theta}(n^2p)$).  This, in turn, implies a lower bound on $|\mathcal{M}|.$ Altogether, this gives the following result.

\begin{theorem}
\label{thm:enumeration}
The number of graphs which can be realized as intersection graphs of unit spheres in dimension $d$ is at least $\exp(nd\log^{-7}n).$     
\end{theorem}

The statement is tight up to the $\log$ terms as shown in \cite{SAUERMANN2021107593}. The result is not new and sharper estimates (up to the log terms) were recently shown in \cite{SAUERMANN2021107593}. Nevertheless, one advantage of our proof is its simplicity - it is based on a natural probabilistic construction, spherical random geometric graphs. The techniques from algebraic geometry and algebraic topology in \cite{SAUERMANN2021107593} are significantly more involved, even though admittedly much more systematic and sharper.

\subsubsection{Inference with Dependent Data: Robust Testing} One immediate application of \cref{thm:stochasticcoupling} is  the following. Suppose that 
$\epsilon\in (0,1]$ is a small fixed constant. Whenever $d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5)$ (where $K(\epsilon)$ depends solely on $\epsilon$), one can with high probability (adversarially) corrupt $\epsilon \binom{n}{2}p$ edges of a sample from $\RGGsphere$ and produce a sample from $\ergraph.$
Hence, the following robust testing problem is information-theoretically impossible when $d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5):$ 
\begin{problem}[Robust Testing of Geometry With Edge Corruptions]
\label{problem:robusttesting}
Given are $n,d\in \mathbb{N},$ $p\in [0,1]$ and a fixed constant $\epsilon.$
Consider the following hypothesis testing problem. One observes a graph $H$ and needs to decide between $H_0: H = \mathcal{A}(\bfG),\bfG\sim \ergraph$ and 
$H_1: H = \mathcal{A}(\bfG),\bfG\sim \mathsf{RGG}(n,d,p).$ Here $\mathcal{A}$ is an arbitrary adversary who is allowed to corrupt at most $\epsilon \binom{n}{2}p$ edges and non-edges.
\end{problem}
We restrict the adversary to changing $\epsilon \binom{n}{2}p$ edges for a small constant $\epsilon$ as the robust testing problem is otherwise trivially impossible. Both $\mathsf{RGG}(n,d,p)$ and 
$\ergraph$ have with high probability $1.5\binom{n}{2}p$ edges. Hence, an adversary $
\mathcal{A}$ who simply deletes all edges of a sample from $\RGG$ and then inserts Bernoulli $p$ edges (in total $3\binom{n}{2}p$ w.h.p.) can transform into a sample from $\ergraph.$ Thus, \cref{problem:robusttesting} captures the setting of ``maximal adversaries.'' 

\begin{remark}[Efficient adversaries]
\label{rmk:eficientadversary}
When $d = o((np)^3(\log n)^3), d\ge K(\epsilon)\max(np (\log n)^{4}, (\log n)^5)),$ \cref{problem:robusttesting} is information theoretically impossible even against polynomial-time adversaries. In this regime, an adversary can see a sample $H$ and (correctly with high probability) test using the signed-triangle statistic \cite{Liu2022STOC} whether the sample is from $\ergraph$ or $\RGGsphere.$ If $H$ is from $\ergraph,$ the adversary can use the efficient algorithm from \cref{thm:algorithmiccoupling} and produce (with high-probability) a sample from $\RGGsphere$ differing from $H$ only at $o\Big(\binom{n}{2}p\Big)$ edges. If $H$ is from $\RGG$ already, the adversary does not change edges. 
\end{remark}



Due to the miraculous coincidence of spectral and entropic thresholds, \cref{problem:robusttesting} is solvable in polynomial time even against computationally unbounded adversaries when $d\ll np.$ 

\begin{theorem}
\label{thm:robustestingsos}
There exists some constant absolute constant $K_r>0$ with the following property. When $d\le K_r\min(np\log(1/p), n^2p^2\log(1/p)\log^{-2}n)$ and $d = \omega(\log 1/p),$ there exists a polynomial-time algorithm solving \cref{problem:robusttesting} with high probability for all $\epsilon\le K_r.$
\end{theorem}
We overview the algorithm in \cref{sec:nontechnicalrobust} and give full detail in \cref{sec:robusttesting}. It is a constant degree SoS program for spectral refutation of a small operator norm of the centered adjacency matrix. The key insight, implicit in \cite{li2023spectral}, is that the latent vectors witness a large second eigenvalue for a random geometric graph. The approach works for robust testing against any null hypothesis with a substantially smaller second eigenvalue than $\RGGsphere,$ see \cref{rmk:testingrobustly}.

\begin{remark}
\label{rmk:couplingimpossibilityfromspectral}
\cref{thm:robustestingsos} implies that when $d \le K_r\min(np\log(1/p), n^2p^2\log(1/p)\log^{-2}n),$ there does not exist a coupling between $H_-\sim \mathsf{G}(n,p(1-o(1)),G\sim \RGGsphere, H_+\sim \mathsf{G}(n,p(1+o(1))$
such that $H_-\subseteq G\subseteq H_+$ w.h.p. Otherwise, one can use this coupling as an adversary for \cref{problem:robusttesting} even against computationally-unbounded testers but \cref{thm:robustestingsos} shows that such an adversary cannot exist. Hence, the dimension requirement $d = \tilde{\Omega}(np)$ in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} is tight (up to $\polylog$ factors).
\end{remark}



\subsection{Prior Work and Challenges}
\paragraph{Coupling Random Geometric Graphs and \ER.} In \cite{Liu2022STOC}, the authors prove \cref{thm:stochasticcoupling} under the weaker condition $d\ge n^2p^2\log^4n.$ In their construction, they sample $V_1, V_2, \ldots, V_n$ sequentially. A caricature of their argument is that with high probability, when sampling $V_1, V_2, \ldots, V_{k-1}$ the intersection of any $i\approx pk$ $p$-caps and $k-i-1\approx k(1-p)$ $p$-anti-caps corresponding to $V_1, V_2, \ldots, V_{i-1}$\footnote{For $V\in \dsphere,$ the associated $p$-cap is the set $\{U \in \dsphere\; : \langle U, V\rangle\ge \tau^p_d\}$  and the $p$-anti-cap is its complement} is sufficiently close to $p^{i}(1-p)^{k-i-1}.$ Hence, one should expect that the edges from $k$ to $[k-1]$ roughly are distributed as ``independent'' $\Bernoulli(p)$ variables. They make this statement precise by quantifying ``sufficiently close'' via a concentration argument based on transportation inequalities. While our proof of \cref{thm:stochasticcoupling} is entirely different, it suggests what might be suboptimal in the approach of \cite{Liu2022STOC}. Typical intersections of $\approx pk$ caps and $k-i-1\approx k(1-p)$ anti-caps might concentrate much better than worst-case 
intersections due to a square-root cancellation phenomenon. We use this idea in our proof to get $d\ge \max(np, \log n)$ and if we consider \emph{all} intersections of caps and anti-caps instead, we also obtain a result for $d\ge n^2p^2\polylog n.$ While the square-root cancellation comes naturally in our martingale-based analysis, it is unclear whether it can be incorporated in the transportation-based approach of \cite{Liu2022STOC}. Even beyond that, an advantage of our approach is that there is an efficient algorithm producing the coupling -- \cref{thm:algorithmiccoupling}. The result of \cite{Liu2022STOC} is not obviously algorithmically efficient as it requires keeping track of an intersection of caps and anti-caps on the sphere and being able to sample and estimate the volume of this intersection.    

A different work which shows that in certain regimes random geometric graphs can be represented as $\ergraph$ with some planted structure (i.e. the edges on locations for which $|\langle V_i, V_j\rangle - \tau_p^d|\le \frac{\sqrt{np\log n}}{d}$ in \cref{thm:algorithmiccoupling}) is 
\cite{bangachev2024fourier}. In fact, in their representation, again the non-\ERspace pairs $(i,j)$ are exactly the ones for which $\langle V_i, V_j\rangle$ are close to $\tau^p_d$ (called \emph{fragile pairs} in \cite{bangachev2024fourier}). While some of our ideas are related to and motivated by \cite{bangachev2024fourier}, there is a fundamental barrier to their proof technique. It crucially relies on performing the Gram-Schmidt operation on the latent vectors\footnote{To be fully precise, the Gram-Schmidt is performed on the isotropic Gaussian vectors $Z_1, Z_2, \ldots, Z_n.$ 
% where $Z_i = V_i \chi_i$ (where $\chi_i$ is an appropriate square root of a $\chi^2$ random variable). 
This, however, makes little difference to the arguments in \cite{bangachev2024fourier} and the current work, see \cref{rmk:sphericaltogaussian}.} $V_1, V_2, \ldots, V_n.$ In particular, this method requires $d\ge n,$ so obtaining a result of the form in \cref{thm:algorithmiccoupling,thm:stochasticcoupling} for $d\ll n$ is impossible. 

\paragraph{Testing.} To the best of our knowledge, this work is the first to study the robust testing problem between $\RGGsphere$ and \ER. The same question in the setting of no edge corruptions has attracted significant attention in recent years \cite{Devroye11,Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC,bangachev2024fourier}. Formally, one observes a graph $G$ and needs to decide $H_0:G\sim \ergraph$ or $H_1:G\sim \RGGsphere.$ By counting signed triangles, i.e computing $\sum_{i<j<k}(G_{ij} - p)(G_{jk}-p)(G_{ki}-p),$ one can succeed with high probability whenever $d = \omega(n^3p^3\log^3(1/p))$ \cite{Bubeck14RGG,Schramm_2022}.  The current state-of-the-art information-theoretic lower bounds are that when $d\ge (\log n)^C n^3p^2,$ the problem is information theoretically impossible as well as when 
$p = \Theta(1/n)$ and $d\ge (\log n)^C$ for some constant $C$ \cite{Liu2022STOC}. Even ignoring $\polylog $ factors, there is still a $1/p$ gap between the testing algorithm and the information-theoretic lower bound when $1/n\ll p\ll 1/2.$ The gap was recently closed with respect to low-degree polynomial tests by \cite{bangachev2024fourier}: counting signed triangles is optimal among all degree $\log^{2-\epsilon} n$ polynomial tests.

We note that both the question of upper and lower-bounds are significantly different when one considers the testing problem with a constant number of adversarial corruptions as in \cref{problem:robusttesting}. On the algorithmic side, simple counting tests such as counting signed triangles necessarily fail. For example, the expected number of signed triangles in $\RGGsphere$ is $\tilde{\Theta}(n^3p^3/\sqrt{d})$ \cite{Liu2022STOC}. One can increase the expected number of signed triangles in $\ergraph$ by planting a clique of size $\tilde{O}(np/d^{1/6})$ which requires $\tilde{O}(n^2p^2/d^{1/3}) = o(n^2p)$ adversarial corruptions. One can argue similarly for other subgraph-counting tests. This is why we need a more sophisticated sum-of-squares spectral refutation algorithm which uses the true embedding as a witness. To the best of our knowledge, \cite{mao2024informationtheoretic} is the only other work which uses an embedding-based approach for testing for random geometric graphs, but their work is in low-dimension and the algorithm is not computationally efficient. Regarding lower-bounds, all of the prior work on the setting without adversarial corruptions \cite{Bubeck14RGG,Brennan19PhaseTransition,Liu2022STOC} very strongly exploits distributional assumptions (such as the relationship to Wishart ensembles and a certain $\KL$-convexity argument revealing the latent vectors). We do not expect that any of these techniques applies to the adversarial setting. Instead, we rely on our coupling argument \cref{thm:stochasticcoupling}.

Finally, there is still a gap between the known upper-bound $\tilde{\Theta}(n^3p^3)$ and the lower-bound $\Tilde{\Theta}(n^3p^2)$ in the setting of no corruptions when $p = \omega(1/n).$ In this work, we determine that (up to log factors) $d = \Tilde{\Theta}(np)$ is the tight threshold for testing with adversarial corruptions computationally and information-theoretically. Part of the reason for this difference between the robust setting and the setting without corruptions is how well we understand the respective thresholds. $d = \Tilde{\Theta}(np)$ has a very clear significance - as an entropic threshold information-theoretically and as a spectral threshold computationally. Yet, the condition $d = \Tilde{\Theta}(n^3p^3)$ so far seems to only have a computational interpretation. It is the threshold below which one can test counting signed triangles, which are ``the most informative subgraph'' among $\log^{2-\epsilon}n$-sized subgraphs \cite{bangachev2024fourier}. The search for the correct information-theoretic interpretation of  $d = \Tilde{\Theta}(n^3p^3)$ remains open.

\paragraph{Sharp Thresholds.} The question of whether monotone properties exhibit sharp thresholds is by far the best understood in the case of product distributions. The seminal paper of \cite{Friedgut1999SharpTO} establishes very broad conditions on vertex-transitive properties for which the \ERspace distribution exhibits sharp-thresholds. In non-product settings, much less is understood. Important progress has been made in the case of measures satisfying the FKG lattice property \cite{grimmett2006random}. However,
this property does not seem to hold obviously for random geometric graphs.
In the case of low-dimensional random geometric graphs (over the solid cube $[0,1]^d$), \cite{goel05monotoneproperties} show sharp-thresholds phenomena by proving that if $G_1, G_2$ are independent samples with densities $p(1-o(1)),p,$ then $G_1\subseteq G_2$ with high probability. The work of \cite{Bradonjic2013OnST} also deals with sharp thresholds on random geometric graphs, but again only applies to low dimensions. The methods of \cite{goel05monotoneproperties,Bradonjic2013OnST} do not seem applicable to the high-dimensional setting because both rely on the fact that a very fine (grid) subdivision of the space is well-covered by the latent vectors. In $d$ dimensions, the subdivision has $\exp(\Omega(d))$ cells, which is much larger than $n$ when $d = \omega(\log n).$
 
To the best of our knowledge, our result is the first to prove a generic sharp-thresholds statement for high-dimensional random geometric graphs in a non-trivial regime (i.e., when $\RGGsphere$ is not asymptotically the product distribution $\ergraph$ in total variation distance). 

\paragraph{Enumeration.} A classic result in algebraic geometry due to Warren \cite{warren1968lowerbounds} nearly immediately implies that the number of geometric graphs in $d$ dimensions is at most $(Cn/d)^{dn}$ for some explicit constant $C$ when $d = o(n)$ \cite{MCDIARMID2011627,SAUERMANN2021107593}. The main idea is that the edges of a geometric graph correspond to the sign patterns of $\binom{n}{2}$ polynomials over the $dn$ variables $\{(v_i)_j\}_{1\le i \le n, 1\le j \le d}.$ The variables are the coordinates of the latent vectors and the polynomials are the squared pairwise $\ell_2$ distance minus the radius squared.

Proving lower bounds, however, turns out to be a much more challenging task. In \cite{MCDIARMID2011627}, it is shown that in 2 dimensions the number of geometric graphs (known also as unit disk graphs in this case) is $n^{(2+o(1))n}.$ Using more sophisticated tools from algebraic geometry and topology, \cite{SAUERMANN2021107593} shows that the number of 
geometric graphs  in $d$ dimensions is $n^{(d+o(1))n}$ when $d = o(n).$

While our proof loses a non-trivial poly-logarithmic factor in the exponent, it is much simpler and relies on a simple probabilistic construction - spherical random geometric graphs.

\paragraph{Other Works on Random Geometric Graphs in The Regime $\log(n)\ll d\ll (np)^3.$} In \cite{Devroye11}, the authors show that as long as $d\gg \polylog(n), $ the clique numbers of $\ergraph$ and $\RGGsphere$ are essentially the same. While their work is also focused on a comparison with \ERspace in a metric other than total variation distance, one major difference is that it is only for a single (monotone) property, the clique number. Our coupling result addresses \emph{all} monotone properties.   

\subsection{Organization}
In \cref{sec:preliminaries} we introduce some basic preliminaries and notation. In \cref{sec:nontechnical}, we give non-technical overviews of our two main algorithmic results: the coupling algorithm in \cref{thm:algorithmiccoupling} and the spectral refutation algorithm in \cref{thm:robustestingsos}. We give the full details in respectively \cref{sec:coupling} and \cref{sec:robusttesting}. In \cref{sec:enumeration} we prove \cref{thm:enumeration} via a rather simple counting argument using \cref{thm:algorithmiccoupling}. We end with several remarks and open questions regarding our results in \cref{sec:discussion}.




==> marginalsoffkg.tex <==
\section{Proof of \texorpdfstring{\cref{claim:marginalsofFKG}}{FKGclaim}}
\label{sec:marginalsoffkg}
We will need the following result from \cite{grimmett06fkg}.

\begin{lemma}
\label{lem:1monotonic}
    A positive measure $\mu$ over $\{0,1\}^N$ satisfies the FKG property if and only if for any $i \in [N]$ and $\xi,\zeta\in \{0,1\}^N$ such that $\xi\le \zeta $ coordinate-wise,
    $$
    \mu(X_i = 1|X_j = \xi_j \; \forall j \neq i)\le 
    \mu(X_i = 1|X_j = \zeta_j \; \forall j \neq i).
    $$
\end{lemma}

\begin{proof}[Proof of \cref{claim:marginalsofFKG}]
Suppose that $\mu$ is a positive measure that satisfies the FKG property. Let $\mu_M$ be its marginal on the first $M$ coordinates. Trivially, $\mu_M$ is positive. To show the fKG property, we use \cref{lem:1monotonic}. Let $i \in [M]$ and let $\xi^M,\zeta^M\in \{0,1\}^M$ be such that $\xi^M\le \zeta^M $ coordinate-wise. We want to show that 
$$
    \mu^M(X_i = 1|X_j = \xi^M_j \; \forall j \neq i, j\in [M])\le 
    \mu^M(X_i = 1|X_j = \zeta^M_j \; \forall j \neq i, j \in [M]).
    $$
    Using the definition of $\mu^M,$ it is enough to show that 
    
\end{proof}
